Concentration of multi-overlaps for random ferromagnetic spin models

We consider ferromagnetic spin models on dilute random graphs and prove that, with suitable one-body infinitesimal perturbations added to the Hamiltonian, the multi-overlaps concentrate for all temperatures, both with respect to the thermal Gibbs average and the quenched randomness. Results of this nature have been known only for the lowest order overlaps, at high temperature or on the Nishimori line. Here we treat all multi-overlaps by a non-trivial application of Griffiths-Kelly-Sherman correlation inequalities. Our results apply in particular to the pure and mixed p-spin ferromagnets on random dilute Erdoes-R\'enyi hypergraphs. On physical grounds one expects that multi-overlap concentration directly implies the correctness of the cavity (or replica symmetric) formula for the pressure. The proof of this formula for the general p-spin ferromagnet on a random dilute hypergraph remains an open problem.

==> sections/argumentsconjectures.tex <==
{\color{blue}
\section{Heuristic Arguments for the Conjectures}\label{willseeifwewrite}
%
In this section we prove the main results of this paper, Theorem \ref{main-thm} and Propositions \ref{bound1}, \ref{bound2}.
For each of these one tries to construct trial distributions that cancel the remainder.

\subsection{Proof of Theorem \ref{main-thm}}

\begin{proposition}[Lower bound]\label{prop:lowerbound}
The replica-symmetric formula is an lower bound to the pressure:
%
\begin{align}\label{thm:ub}
\liminf_{n \rightarrow \infty} p_n \geq {\adjustlimits \sup_{\sfx \in \mathcal{P}} \inf_{\tilde{\sfx} \in \tilde{\mathcal{P}}} p_{\mathrm{RS}}(\sfx, \tilde{\sfx})} \,.
\end{align}
\end{proposition}

\begin{proof}
From \eqref{remainderhasbeencancelled} we deduce
\begin{align}\label{56}
p_n \geq \inf_{\tilde{\underline{\sfx}}\in \tilde{\mathcal{P}}^{T_n}} p_{T_n}( \{\sfx_{n}\}_{t=0}^{T_n}, \{\tilde{\sfx}_n^{(t)}[\sfx_n]\}_{t=0}^{T_n} ; 0, 0) + \smallO_n(1)
\end{align}
In Appendix \ref{proof:h_RS_coupled:equivalence} we remark that the functional 
$\tilde{\underline\sfx}\in \tilde{\mathcal{P}}^{T_n} \mapsto p_{T_n}( \{\sfx_{n}\}_{t=0}^{T_n}, \tilde{\underline{\sfx}} ; 0, 0)\in \mathbb{R}$ depends $\tilde{\underline{\sfx}}$ only through the mean
$T^{-1}\sum_{t=1}^{T_n} \tilde{\sfx}^{(t)}$. Therefore \eqref{56} implies
%
\begin{align}
p_n & \geq \inf_{\tilde{\underline{\sfx}}\in \tilde{\mathcal{P}}^{T_n}} p_{T_n}( \{\sfx_{n}\}_{t=0}^{T_n}, \{\tilde{\sfx}_n^{(t)}[\sfx_n]\}_{t=0}^{T_n} ; 0, 0) + \smallO_n(1)
\nonumber \\ &
\geq \inf_{\tilde{\sfx}\in \tilde{\mathcal{P}}} p_{T_n}( \{\sfx_{n}\}_{t=0}^{T_n}, \{\tilde{\sfx}_n\}_{t=0}^{T_n} ; 0, 0) + \smallO_n(1)
\nonumber \\ &
= \inf_{\tilde{\sfx}\in \tilde{\mathcal{P}}} p_{\rm RS}(\sfx_{n}, \tilde{\sfx}) + \smallO_n(1)
\end{align}
%
Since $\sfx_n$ is arbitrary we can optimize on it, to obtain
%
\begin{align}
p_n \geq 
\sup_{\sfx\in \mathcal{P}}\inf_{\tilde{\sfx}\in \tilde{\mathcal{P}}} p_{\rm RS}(\sfx, \tilde{\sfx}) + \smallO_n(1)
\end{align}
%
which implies the statement of the proposition by taking the liminf.
\end{proof}

We now turn to the converse bound.

\begin{proposition}[Upper bound]\label{prop:upperbound}
The replica-symmetric formula is an upper bound to the pressure:
%
\begin{align}\label{thm:ub}
\limsup_{n \rightarrow \infty} p_n \leq {\adjustlimits \sup_{\sfx \in \mathcal{P}}\inf_{\tilde{\sfx} \in \tilde{\mathcal{P}}} 
p_{\mathrm{RS}}(\sfx, \tilde{\sfx})} \,.
\end{align}
\end{proposition}
%
\begin{proof}
We first note that by a convexity inequality in Appendix \ref{proof:h_RS_coupled:equivalence} equation \eqref{remainderhasbeencancelled} implies
%
\begin{align}\label{startingpoint}
p_n \leq 
\frac{1}{T_n}\sum_{t=1}^{T_n}
p_{\rm RS}(\sfx_{n}, \tilde{\sfx}_n^{(t)}[\sfx_n]) + \smallO_n(1)\,.
\end{align}
%
We choose $\sfx_n = \sfx_{n,*}^{(t)}$ where $\sfx_{n,*}^{(t)}$ is the solution of the fixed point equation (equality the sense of distributions)
\begin{align}\label{statpointVU}
V_n^{(t)} \overset{d}{=} H + \sum_{b=1}^{l-1} U_{n, b}^{(t)}
\end{align}
where $V_n^{(t)}\sim \sfx_{n,*}^{(t)}$, $U_{n, b}^{(t)}\sim \tilde{\sfx}_n^{(t)}[\sfx_{n,*}^{(t)}]$ for $b=1, \cdots, l-1$ and $l\sim {\rm Poi}(\gamma p)$. The existence of $\sfx_{n,*}^{(t)}$ is ensured by Schauder's fixed point theorem as shown in Appendix \ref{schauder-fix-point}. Now, note that \eqref{statpointVU} is the stationary point equation of the functional 
$\tilde\sfx \in \tilde{\mathcal{P}} \mapsto p_{\rm RS}(\sfx_{n,*}^{(t)}, \tilde{\sfx})\in \mathbb{R}$ and that this this functional is convex on the convex set $\tilde{\mathcal{P}}$. 
Thus $\tilde{\sfx}_n^{(t)}[\sfx_{n,*}]$ must be a minimizer of $p_{\rm RS}(\sfx_{n,*}^{(t)}, \tilde{\sfx})$
and \eqref{startingpoint} yields
\begin{align}
p_n 
& 
\leq 
\frac{1}{T_n}\sum_{t=1}^{T_n}
p_{\rm RS}(\sfx_{n,*}^{(t)}, \tilde{\sfx}_n^{(t)}[\sfx_n]) + \smallO_n(1)
\nonumber \\ &
= 
\frac{1}{T_n}\sum_{t=1}^{T_n}
\inf_{\tilde{\sfx}\in \tilde{\mathcal{P}}} p_{\rm RS}(\sfx_{n,*}^{(t)}, \tilde{\sfx}) + \smallO_n(1)\, .
\end{align}
Finally,
\begin{align}
p_n \leq \sup_{\sfx\in \mathcal{P}}\inf_{\tilde{\sfx}\in \tilde{\mathcal{P}}} p_{\rm RS}(\sfx, \tilde{\sfx}) + \smallO_n(1)
\end{align}
and taking the limsup completes the proof. 
\end{proof}


\subsection{Proof of of lower bound in proposition \ref{bound1}}\label{proofbound1}
%
For each $T_n$ we consider some trial distribution $\tilde\sfx_n\in \tilde{\mathcal{P}}$ and set $\tilde\sfx^{(t)} = \tilde\sfx_n$, $t=1,\cdots, T_n$.
We choose $\{{\sfx}_n^{(t)}\}_{t=1}^{T_n} \in \mathcal{P}^{T_n}$ to be the solution of the equations
\begin{align}\label{firstequation}
 q_{n,k}^{(t)} = \mathbb{E}\langle Q_k\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}} \quad {\rm for} \quad  k\geq 1,\quad  t=1,\cdots, T_n.
\end{align}
In order to check that there exist such $\underline {\sfx}_n$ we must verify that there exist random variables $V_n^{(t)}$, $t=1,\cdots, T_n$ such that \eqref{firstequation} holds (recall the definition \eqref{def:qs}). 
First notice 
that by construction of the interpolating Hamiltonian \eqref{eq:Hamiltonian_ts}, \eqref{eq:Hamiltonian_tse} the Gibbs bracket \eqref{productmeasure} does {\it not} depend on $\tanh V^{(t)}$, $t=1, \cdots, T_n$. 
Therefore the only thing we should check is that the set of numbers $\mathbb{E}\langle Q_k\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}$, $k\geq 1$ correspond to the moments of a $[0,1]$-valued random variable. 
But this is trivially so by 
the very definition of these numbers (we can also assert that the solution is unique because this is a Haussdorff moment problem but unicity is not needed for the argument).
We call $\{{\sfx}_{n}^{(t)}[\tilde{\sfx}_{n}]\}_{t=1}^{T_n}$ 
the solution. 
From \eqref{second-simplif}, \eqref{Rhat-s=0} we obtain
\begin{align}
p_n  = {p}_{T_n}(\{{\sfx}_{n}^{(t)}[\tilde{\sfx}_{n}]\}_{t=1}^{T_n}, \{\tilde{\sfx}_n\}_{t=0}^{T_n}; 0,0) + \smallO_n(1).
\end{align}
This implies the lower bound
\begin{align}\label{onestep}
 p_n  \geq \inf_{\underline{\sfx}\in \mathcal{P}^{T_n}} p_{T_n}(\underline{\sfx}, \{{\tilde{\sfx}}_n\}_{t=0}^{T_n}; 0,0) + \smallO_n(1).
\end{align}
In Appendix \ref{proof:h_RS_coupled:equivalence} we show that the functional $\underline \sfx \mapsto p_{T_n}(\underline{\sfx}, \{{\tilde{\sfx}}_n\}_{t=0}^{T_n}; 0,0)$ satisfies 
\begin{align}\label{twostep}
 p_{T_n}(\underline{\sfx}, \{{\tilde{\sfx}}_n\}_{t=0}^{T_n}; 0,0) = \frac{1}{T_n}\sum_{t=1}^{T_n} p_{\rm RS}\big(\sfx^{(t)}, \tilde{\sfx}_n\big)\,.
\end{align}
From \eqref{onestep}, \eqref{twostep} 
\begin{align}
 p_n \geq \inf_{\sfx\in \mathcal{P}}p_{\rm RS}(\sfx, \sfx_n) +\smallO_n(1)
\end{align}
and optimizing over $\sfx_n$ we get
\begin{align}
p_n \geq \sup_{\tilde{\sfx}\in \tilde{\mathcal{P}}}\inf_{\sfx\in \mathcal{P}}p_{\rm RS}(\sfx, \tilde{\sfx}) +\smallO_n(1)
\end{align}
taking the liminf completes the proof.

\subsection{The case of the Ising model $p=2$}

Here we derive the converse bound to Proposition \ref{bound1} for $p=2$. It is not clear how to proceed for higher $p$ (see remark below). 
Recall $U^{(t)}\sim \tilde{\sfx}^{(t)}$ and $V^{(t)}\sim \sfx^{(t)}$. 
We take a fixed $\tilde{\sfx}_n^{(t)}\in \tilde{\mathcal{P}}$ and define ${\sfx}_n^{(t)}[\tilde{\sfx}_n^{(t)}]$ such that
\begin{align}
 \tanh U^{(t)}_n \overset{d}{=} (\tanh \tJ) \tanh V_{n}^{(t)}, \qquad t=1, \cdots, T_n\,.
\end{align}
This implies
\begin{align}
\tilde{q}_{n,k}^{(t)} = (\tanh \tJ)^k q_{n,k}^{(t)} \quad {\rm for} \quad k\geq 1, \,  t=1,\cdots,T_n\,
\label{eq:fixed-qt}
\end{align}
so \eqref{second-simplif}, \eqref{Rhat-s=0} become
%
\begin{align}\label{third-simplif}
p_n  = & {p}_{T_n}(\{{\sfx}_n^{(t)}[\tilde{\sfx}_n^{(t)}]\}_{t=0}^{T_n}, \{\tilde{\sfx}_n^{(t)}\}_{t=0}^{T_n} ; 0,0) 
\nonumber \\ &
+ \frac{\gamma}{T_n} \sum_{t=1}^{T_n}\sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k (\tanh J)^k}
\big((\tanh J)^k\mathbb{E}[\langle Q_{k}\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}]  - \tilde{q}_{n,k}^{(t)}\big)^2 + \smallO_n(1)\,.
\end{align}
%
In order to cancel the remainder we want to find random variables $U_n^{(t)}$ that satisfy
\begin{align}\label{stillamoment}
 \tilde{q}_{n,k}^{(t)} = (\tanh J)^k\mathbb{E}[\langle Q_{k}\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}],\qquad k\geq 1, \, t=1, \cdots, T_n\,.
\end{align}
Since $\langle - \rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}$ depends only on $U_n^{(1)}, \cdots, U_n^{(t-1)}$ and not on $U_n^{(t)}, \cdots, U_n^{(T_n)}$ this moment problem can be solved recursively. Let 
$\tilde{\underline\sfx}_{n,*}$ be the distribution that solves \eqref{stillamoment}. We have 
\begin{align}\label{pasmarrant}
 p_n  =  {p}_{T_n}(\{{\sfx}_n^{(t)}[{\tilde{\sfx}}_{n,*}^{(t)}]\}_{t=0}^{T_n}, \{{\tilde{\sfx}}_{n,*}^{(t)}\}_{t=0}^{T_n}; 0,0)  + \smallO_n(1)\,.
\end{align}
By a convexity inequality in Appendix \ref{proof:h_RS_coupled:equivalence} we have 
\begin{align}\label{pasmarrant}
 p_n  \leq  \frac{1}{T_n}\sum_{t=1}^{T_n} 
 p_{\rm RS}({\sfx}_n^{(t)}[{\tilde{\sfx}}_{n,*}^{(t)}], {\tilde{\sfx}}_{n,*}^{(t)})  + \smallO_n(1)\,.
\end{align}
Now, consider the functional $\sfx\in \mathcal{P} \mapsto {p}_{\rm RS}(\sfx, \tilde{\sfx}_{n,*}^{(t)})\in \mathbb{R}$. 
It is not difficult to see that: (i) ${\sfx}_n^{(t)}[\tilde{\sfx}_{n, *}^{(t)}]$ is a stationary point and; (ii)
the functional is convex over the convex set $\mathcal{P}$ (see Appendix \ref{proof:h_RS_coupled:equivalence}). Therefore 
$\sfx_n^{(t)}[\tilde{\sfx}_{n,*}^{(t)}]$ is a minimizer of this functional and therefore \eqref{pasmarrant} becomes 
\begin{align}
 p_n  & \leq  \frac{1}{T_n}\sum_{t=1}^{T_n} 
 \inf_{\sfx\in \mathcal{P}}p_{\rm RS}(\sfx, {\tilde{\sfx}}_{n,*}^{(t)})  + \smallO_n(1)
 \nonumber \\ &
 \leq 
 \sup_{\tilde\sfx \in \tilde{\mathcal{P}}}\inf_{\sfx\in \mathcal{P}}p_{\rm RS}(\sfx, \tilde{\sfx}) + \smallO_n(1)\,.
\end{align}
Taking the lim completes the proof. 
}


%
% These equations indeed possess at least a solution. This is guaranteed by the following lemma:
% \begin{lemma}[Existence of the optimal interpolation path]
% For all $n\in \mathbb{Z}_{\ge 1}$ there exists at least one solution $\underline{\sfx}^* \in \mathcal{P}^T$ for equations \eqref{eq:momentMatching:ub}.
% \label{thm:momentMatching:solution-ub}
% \end{lemma}
% \begin{proof}
% By symmetry all spins are statistically equivalent, therefore $\mathbb{E}\langle Q_k \rangle_{t,0; h_n, \alpha_n} = \mathbb{E}[\langle \sigma_1 \rangle_{t,0; {h}_n, \alpha_n}^k]$. Recall definition \eqref{def:qs}. A solution $\underline{\sfx}^*=\{\sfx^{(t),*}\}_{t=1}^T$ for \eqref{eq:momentMatching:ub} is as follows: For $t=1,\ldots,T$ let $V^{(t)}\sim \sfx^{(t),*}$ and such that $\tanh V^{(t)}$ is distributed as $\< \sigma_1 \>_{t,0; {h}_n, \alpha_n}$. The GKS inequality \eqref{eq:GKS1} tells $\< \sigma_1 \>_{t,0; {h}_n, \alpha_n} \geq 0$, thus $\sfx^{(t),*} \in \mathcal{P}$.	
% \end{proof}
% %
% This solution $\underline{\sfx}^*$ of \eqref{eq:momentMatching:ub} cancels the sum over $k$ in \eqref{eq:interpolation:remainder-ub} and thus, when used in conjunction with \eqref{eq:interpolation:main2-ub}, yields
% \begin{align}
% \limsup_{n \rightarrow \infty} f_{1,0; {h}_n, \alpha_n} = \lim_{n \rightarrow \infty} {f}_{{\rm RS};{h}_n, \alpha_n} (\underline{\sfx}^*, \underline{\sfx}^{\dagger}(\underline{\sfx}^*))\,.
% \label{eq:feqtf2}
% \end{align}
% %
% As $h_n\to0_+$ Lemma \ref{rmk35} can then used to turn \eqref{eq:feqtf2} into
% \begin{align}
% \limsup_{n \rightarrow \infty} f_{1,0; {h}_0=0, \alpha=0} = {f}_{{\rm RS};{h}_0=0, \alpha=0} (\underline{\sfx}^*, \underline{\sfx}^{\dagger}(\underline{\sfx}^*))\,. \label{44}
% \end{align}
% At this stage we note that, by definition \eqref{xdagger} of $\underline{\sfx}^{\dagger}(\underline{\sfx}^*)$, the right hand side of the previous inequality can be bounded as 
% \begin{align*}
% {f}_{{\rm RS};{h}_0=0, \alpha=0}(\underline{\sfx}^*, \underline{\tilde{\sfx}}^\dagger(\underline{\sfx}^*) ) 
% 	= \inf_{\underline{\tilde{\sfx}} \in \tilde{\mathcal{P}}^T} {f}_{{\rm RS};{h}_0=0, \alpha=0}(\underline{\sfx}^*, \underline{\tilde{\sfx}}) 
% 	\leq {\adjustlimits \sup_{\underline{\sfx} \in \mathcal{P}^T} \inf_{\underline{\tilde{\sfx}} \in \tilde{\mathcal{P}}^T}} {f}_{{\rm RS};{h}_0=0, \alpha=0}(\underline{\sfx}, \underline{\tilde{\sfx}}) 
% 	= {\adjustlimits \sup_{\sfx \in \mathcal{P}} \inf_{\tilde{\sfx} \in \tilde{\mathcal{P}}}} f_{\mathrm{RS}}(\sfx, \tilde{\sfx})
% \end{align*}
% where the last equality follows from Lemma~\ref{lemma:3.2}. Finally use \eqref{20} to replace the left hand side of \eqref{44} to finish the proof of Proposition \ref{prop:upperbound}.
% 





==> sections/cancellingremainder.tex <==
\section{Proof of the Replica Symmetric Variational Bound}\label{cancelling}
%
In this section we explore the consequences of the sum rule \eqref{second-simplif} and \eqref{Rhat-s=0}. The general philosophy of the approach is to cancel the remainder 
\eqref{Rhat-s=0} by a suitable choice of the trial distributions. When this can be done matching bounds on the pressure can often be derived as shown in \cite{matrix}, \cite{tensor}, \cite{perceptron}, \cite{GLM}.
For the ferromagnetic model on a sparse graph it turns out that this last step presents new difficulties that we discuss in Section \ref{subsec:discussion}. 

\subsection{Proof of Proposition \ref{bound2}}\label{proofbound2}

The bound that we want to prove here involves only an optimization over $\sfx\in \mathcal{P}$. We therefore start by expressing the interpolating Hamiltonian entirely in terms 
of the random variables $V^{(t)}\sim \sfx^{(t)}$. Fix a trial distribution $\underline\sfx_n\in \mathcal{P}^{T_n}$ and let $V_n^{(t)}\sim \sfx_n^{(t)}$. Take $p-1$ iid copies $V_{n,j}^{(t)}$, $j=1, \cdots, p$ and define
\begin{align}\label{Uinduced}
 \tanh U_n^{(t)} \overset{d}{=} \tanh J\prod_{j=1}^{p-1} \tanh V_{n,j}^{(t)} \qquad t=1, \cdots, T_n
\end{align}
The distribution of \eqref{Uinduced} is denoted $\tilde{\sfx}_n^{(t)}[\sfx_n^{(t)}]$ emphasizing that it is entirely determined by $\sfx_n^{(t)}$.
The Gibbs bracket $\langle - \rangle_{t, 0; h_0^{(n)}, \alpha^{(n)}}$ now depends on $V^{(1)}, \cdots, V^{(t-1)}$. Note for further use that it is independent of 
$V^{(t)}, \cdots, V^{(T_n)}$. Furthermore we have 
\begin{align}
\mathbb{E}[(\tanh U_n^{(t)})^k] = (\tanh \tJ)^k (\mathbb{E}[(\tanh V_n^{(t)})^k])^{p-1} \qquad  t=1,\cdots,T_n
\end{align}
or equivalently
\begin{align}
\tilde{q}_{n,k}^{(t)} = (\tanh \tJ)^k (q_{n,k}^{(t)})^{p-1} \qquad t=1,\cdots,T_n\, .
\label{eq:fixed-qt}
\end{align}
and \eqref{second-simplif}, \eqref{Rhat-s=0} become
%
\begin{align}
p_n  = & p_{T_n}(\{{\sfx}_n^{(t)}\}_{t=1}^{T_n}, \{{\tilde\sfx}_n^{(t)}[\sfx_n^{(t)}]\}_{t=1}^{T_n}; 0,0) + \frac{\gamma}{T_n} \sum_{t=1}^{T_n}\sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} (\tanh \tJ)^{k}\biggl\{  
\big(\mathbb{E}[\langle Q_{k}\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}]^p  - q_{n,k}^{(t) p}\big) 
\nonumber \\ &
- p q_{n,k}^{(t) p-1}\big(\mathbb{E}[\langle Q_k\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}]  - q_{n,k}^{(t)} \big)\biggr\} + \smallO_n(1)
\end{align}
Now we seek a solution  to the equation
\begin{align}\label{cancellinGT}
 q_{n,k}^{(t)} = \mathbb{E}[\langle Q_k\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}], \quad k\geq 1, \, t=1, \cdots, T_n\,.
\end{align}
We must verify that there exist random variables $V_n^{(t)}$ such that the right hand side equals $\mathbb{E}[(\tanh V_{n}^{(t)})^k]$. Since the Gibbs bracket depends only on 
$V^{(1)}, \cdots, V^{(t-1)}$ it is clear that these random variables are constructed recursively. We call ${\sfx}_{n,*}^{(t)}$ the solution of \eqref{cancellinGT}. Then 
\begin{align}\label{one}
 p_n  & =  p_{T_n}(\{{\sfx}_{n,*}^{(t)}\}_{t=1}^{T_n}, \{{\tilde\sfx}_n^{(t)}[\sfx_{n,*}^{(t)}]\}_{t=1}^{T_n}; 0,0) + \smallO_n(1)
\end{align}
Then from the definition of $p_T^{(1)}(\underline\sfx)$ we immediately get
\begin{align}
 p_n \leq p_{T_n}^{(1)}(\{{\sfx}_{n,*}^{(t)}\}_{t=1}^{T_n}) \le \sup_{\underline \sfx\in \mathcal{P}^{T_n}} p_{T_n}^{(1)}(\underline \sfx) + \smallO_n(1)
\end{align}
which is the statement of Proposition \ref{bound2}.

% In Appendix \eqref{proof:h_RS_coupled:equivalence} we show  a convexity inequality which we apply here as 
% \begin{align}
%  p_{T_n}(\{{\sfx}_{n,*}^{(t)}\}_{t=0}^{T_n}, \{{\tilde\sfx}_n^{(t)}[\sfx_{n,*}^{(t)}]\}_{t=0}^{T_n}; 0,0) & \leq \frac{1}{T_n}\sum_{t=1}^{T_n} p_{\rm RS}^{(1)}(\sfx_{n,*}^{(t)}, {\tilde\sfx}_n^{(t)}[\sfx_{n,*}^{(t)}])
%  \nonumber \\ &
%  = 
%  \frac{1}{T_n}\sum_{t=1}^{T_n} p_{\rm RS}^{1)}(\sfx_{n,*}^{(t)})\,.
%  \label{two}
% \end{align}
% where the equality comes from the definition of $p_{\rm RS}(\sfx)$ in Sec. \ref{rsresults}. From \eqref{one}, \eqref{two}
% \begin{align}
%  p_n \leq \sup_{\sfx\in \mathcal{P}^{T_n}} p_{\rm RS}^{(1)}(\sfx) + \smallO_n(1)
% \end{align}



% In Appendix \eqref{proof:h_RS_coupled:equivalence} we show  a convexity inequality which we apply here as 
% \begin{align}
%  p_{T_n}(\{{\sfx}_{n,*}^{(t)}\}_{t=0}^{T_n}, \{{\tilde\sfx}_n^{(t)}[\sfx_{n,*}^{(t)}]\}_{t=0}^{T_n}; 0,0) & \leq \frac{1}{T_n}\sum_{t=1}^{T_n} p_{\rm RS}^{(1)}(\sfx_{n,*}^{(t)}, {\tilde\sfx}_n^{(t)}[\sfx_{n,*}^{(t)}])
%  \nonumber \\ &
%  = 
%  \frac{1}{T_n}\sum_{t=1}^{T_n} p_{\rm RS}^{1)}(\sfx_{n,*}^{(t)})\,.
%  \label{two}
% \end{align}
% where the equality comes from the definition of $p_{\rm RS}(\sfx)$ in Sec. \ref{rsresults}. From \eqref{one}, \eqref{two}
% \begin{align}
%  p_n \leq \sup_{\sfx\in \mathcal{P}^{T_n}} p_{\rm RS}^{(1)}(\sfx) + \smallO_n(1)
% \end{align}
% which is the statement of Proposition \ref{bound2}.

%In this section we prove the main results of this paper, Theorem \ref{main-thm} and Propositions \ref{bound1}, \ref{bound2}.
%For each of these one tries to construct trial distributions that cancel the remainder.

\subsection{Another cancellation method for the remainder}

The first step is to cancel the remainder \eqref{Rhat-s=0}.
Fix a sequence of trial distributions $\sfx_n \in \mathcal{P}$ and set $\sfx^{(t)} = \sfx_n$ for all $t=1, \cdots, T_n$. In Lemma 
\ref{diffequsol} below we construct a distribution
$\tilde{\underline{\sfx}}_n[\sfx_n]\in \tilde{\mathcal{P}}^{T_n}$ satisfying
%
\begin{align}
(\tanh \tJ)^{k} \big(\mathbb{E}[ \< Q_{k} \>_{t,0; h_n, \alpha_n}  ]^{p} - q_{n,k}^{p} \big) - p\, \tilde{q}_{n,k}^{(t)} \big( \mathbb{E} \< Q_k \>_{t,0; h_n, \alpha_n} - q_{n,k} \big) = 0 
\label{eq:momentMatching:lb}
\end{align}
%
for all $k\geq 1$ and $t=1, \cdots, T_n$. In this equation $q_{n,k} = \mathbb{E}[(\tanh V_n)^k]$, $V_n \sim \sfx_n$, 
$\tilde q_{n,k}^{(t)} = \mathbb{E}[(\tanh U_n^{(t)})^k]$, $U_n^{(t)} \sim \tilde{\sfx}^{(t)}[\sfx_n]$. Then \eqref{second-simplif} becomes
%
\begin{align}\label{remainderhasbeencancelled-firststep}
p_n = p_{T_n}( \{\sfx_{n}\}_{t=1}^{T_n}, \{\tilde{\sfx}_n^{(t)}[\sfx_n]\}_{t=1}^{T_n}; 0, 0) + \smallO_n(1)
\end{align}
%
It can be shown that the dependence in $\{\tilde{\sfx}_n^{(t)}[\sfx_n]\}_{t=1}^{T_n}$ effectively enters as $\frac{1}{T}\sum_{t=1}^{T_n} \tilde\sfx_n^{(t)}[\sfx_n]$ and that therefore 
\begin{align}\label{remainderhasbeencancelled}
p_n = p_{\rm RS}^{(2)}( \sfx_{n}, \frac{1}{T}\sum_{t=1}^{T_n} \tilde{\sfx}_n^{(t)}[\sfx_n]) + \smallO_n(1)
\end{align}


\begin{lemma}[Existence of the solution of \eqref{eq:momentMatching:lb}]\label{diffequsol}
Take a sequence $\sfx_n\in \mathcal{P}$ and set  $\sfx^{(t)} = \sfx_n$ for all $t=1, \cdots, T_n$. There exist $\tilde{\underline{\sfx}}_n[\sfx_n]\in \tilde{\mathcal{P}}^{T_n}$
which is a solution to \eqref{eq:momentMatching:lb}.
\end{lemma}

\begin{proof}
We must show there exist $U_n^{(t)}$ such that for $t=1, \cdots, T_n$ 
\begin{align}
\tilde{q}_{n,k}^{(t)}
	& = \frac{(\tanh J)^k \big( \mathbb{E}[\<Q_k\>_{t,0; {h}_n, \alpha_n}]^p - q_{n, k}^p \big)}{p \big ( \mathbb{E}\<Q_k\>_{t,0; {h}_n, \alpha_n} - q_{n,k}\big )} \-
	= (\tanh J)^k\frac{1}{p} \sum_{r=0}^{p-1} \mathbb{E}[\<Q_k\>_{t,0; {h}_n, \alpha_n}]^{p-1-r} q_{n,k}^r \,.
\end{align}
%
or equivalently using $\mathbb{E}\langle Q_k \rangle_{t,0; {h}_n, \alpha_n} = \mathbb{E}[\langle \sigma_1 \rangle_{t,0; {h}_n, \alpha_n}^k]$ by symmetry among spins
%
\begin{align}
\mathbb{E} [(\tanh U_n^{(t)})^k] = (\tanh J)^k \frac1p\sum_{r=0}^{p-1} \mathbb{E}[\langle \sigma_1 \rangle_{t,0; {h}_n, \alpha_n}^k]^{p-1-r} \, \mathbb{E} [(\tanh V_n)^k]^r\,.
\label{33simple}
\end{align}
%
First we note that from the construction of the interpolating Hamiltonian \eqref{eq:Hamiltonian_ts} the Gibbs bracket $\langle - \rangle_{t,0; {h}_n, \alpha_n}$ depends on $U^{(1)}, \cdots, U^{(t-1)}$ but not on $U^{(t)}, \cdots, U^{(T_n)}$. Therefore $U^{(t)}$ is constructed recursively, as long as we can guarantee that the right hand side of this equation is equal to a moment of a $[0,1]$-valued random variable. Once this existence question is settled we also know that the solution is unique by standard theory of the (Hausdorff) moment problem. We present a constructive proof of existence: 
%
\begin{enumerate}
\item Uniformly pick an $r \in \{1,\dots, p\}$;
\item Create $p-1-r$ {\it independent} graphs from the ensemble $\sG_{t,0}$ and $p-1-r$ independent random 
Gibbs brackets $\langle - \rangle^{(j)}_{t, 0; h_0^{(n)}, \alpha^{(n)}}$, $j=1, \cdots, p-1-r$ (these are not to be confused with the replicas entering the product measure and which share the same quenched randomness); 
%such that the variable $\sigma_1$ in each graph is denoted by $\sigma_{1}^{[1]}, \ldots, \sigma_{1}^{[p-1-r]}$ (not to be confused with replicas $\sigma_1^{(1)}$, $\sigma_1^{(2)}$, $\ldots$ that share in common the quenched variables and underlying graph, while $\sigma_{1}^{[1]}$, $\sigma_{1}^{[2]}$, $\ldots$ are totally independent);
\item Create $r$ i.i.d. copies $V_{n,i}$, $i=1, \cdots, r$ of $V_n\sim \sfx_n$;
\item Set in distribution 
$\tanh U_n^{(t)}\overset{d}{=}\tanh \tJ \prod_{j=1}^{p-1-r} \<\sigma_1\>_{t,0; {h}_n, \alpha_n} \prod_{i=1}^{r} \tanh V_{n,i}$.
\end{enumerate}
%
Since $0\le\<\sigma_1\>\le 1$ by GKS we have $0 < \tanh U^{(t)} <\tanh J$ so $\tilde{\sfx}_n^{(t)}[\sfx_n] \in \tilde{\mathcal{P}}$. Moreover 
one immediately sees that the moments satisfy \eqref{33simple}.
\end{proof}

\subsection{discussion}\label{subsec:discussion}

For the $p$-spin model on a complete hypergraph (for $p=2$ this is simply the Curie-Weiss model) the analog of equation \eqref{remainderhasbeencancelled} forms the basis for deducing matching lower and upper bounds on the pressure 
and thereby providing a (new) proof of the mean field solution. A pedagogic review of this approach can be found in \cite{ourCurieWeisspaper}. But the same proof technique often works also in much more challenging situations, and notably in many inference problems. 
For example, the approach has been successfuly developed for matrix and tensor factorization \cite{bla}, \cite{bla}, generalized linear estimation and perceptron learning \cite{bla}, all in a 
teacher-student setting where an underlying  ground truth is present\footnote{For the assortative Stochastic Block Model however, which is also an inference problem with an underlying round truth, there are difficulties of the same nature discussed here for the 
ferromagnetic $p$-spin dilaute model. Therefore one should not be tempted to conjecture that the approach works for all inference problems.}.

We wish here to briefly discuss the nature of the difficulties encountered in the case of a dilute $p$-spin ferromagnetic model. Let us begin with a lower bound on the pressure that immediately follows from \eqref{remainderhasbeencancelled}.
Clearly for each fixed $\sfx_n\in \mathcal{P}$ we have 
\begin{align}
 p_n & = p_{T_n}( \{\sfx_{n}\}_{t=1}^{T_n}, \{\tilde{\sfx}_n^{(t)}[\sfx_n]\}_{t=1}^{T_n}; 0, 0)  + \smallO_n(1)
 \nonumber \\ &
 \geq \inf_{\tilde{\sfx}\in\mathcal{P}} p_{\rm RS}^{(2)}(\sfx_{n}, \tilde{\sfx}) +\smallO_n(1)
\end{align}
Since $\sfx$ is arbitrary we can tighten the inequality on the rhs to get
\begin{align}
 \liminf_{n\to +\infty} p_n \geq \sup_{\sfx\in \mathcal{P}}\inf_{\tilde{\sfx}\in\mathcal{P}} p_{\rm RS}^{(2)}(\sfx_{n}, \tilde{\sfx})\,.
\end{align}
Unfortunately it is not clear wether this inequality is tight or not for the $p$-spin model on a dilute graph. 

{\color{blue} To derive a converse bound one can choose $x_n^*$ such that... I have to think...}







==> sections/concentrationofmultioverlaps.tex <==
\section{Concentration of the multi-overlaps}\label{sec:cancelR}
%
%
The next step is to exploit a powerful concentration result for the multi-overlaps which is at the heart of teh replica symmetric behavior of the model. 
The proof of the following theorem is based on the GKS correlation inequalities and the concentration of the pressure 
$P_{n, t,s}(h_0, \alpha)$ (for the interpolated model) is deferred to Sec.~\ref{sec:conc}.
%
\begin{theorem}[Multi-overlap concentration]\label{prop:conc_overlap}
For the interpolating model, all multi-overlaps \eqref{def:overlap} concentrate around their mean
$\mathbb{E}[\<Q_k\>_{t,s; h_0, \alpha}]$.
More precisely we consider the perturbed interpolating model with $\theta\in (1/2, 5/6)$, $0 < h_0 <1$ and $0<\alpha <1$. One can find a constant $C(p, J)>0$  
(depending only on $p$ and $J$) such that for any $k\geq 1$,
$0 <\underline h < \bar h < 1$, $0 < \underline \alpha <\bar \alpha<1$ we have
\begin{align}\label{concmultiover}
\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0\,\mathbb{E} \big\< \big| Q_k^p 
- \mathbb{E}[\<Q_k\>_{t,s; h_0, \alpha}]^p \big| \big\>_{t,s; h_0, \alpha} 
\leq \frac{k}{(\tanh h_1)^{k/2}} \frac{C(p, J)}{n^{1/12}}\,.
\end{align}	
\end{theorem}
%
%%%%%%%%%%%%%%%%%%%%DO NOT ERASE%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% {\color{blue} Rewrite. Let us open a parenthesis and discuss various existing results on overlaps concentration. When such concentration does not occur, more complex formulas can be derived thanks to the so-called replica-symmetry broken cavity and replica methods (that are equivalent) \cite{mezard1990spin}. Such scheme has been developed by Giorgio Parisi in order to derive the free energy of the Sherrington-Kirkpatrick model of spin glass. The famous Parisi formula has then been proven by Michel Talagrand \cite{talagrand2006parisi,talagrand2010meanfield1,talagrand2010meanfield2}, where one of his bound follows from the replica-symmetry broken interpolation developed by Francesco Guerra in \cite{guerra2003broken}, the other from the Aizenman-Sims-Starr scheme \cite{aizenman2003extended}. See also the very nice book by Dmitry Panchenko for an alternative simpler proof of the Parisi formula and a quite complete review of the associated proof techniques \cite{Panchenko2013}.
% Let us mention that in dense systems, where variables interact with $\Theta(n)$ other ones, the Gibbs-Boltzmann measure of the model, and thus all its physics, is fully controlled by the overlap $Q_2$ between two replicas only; the higher order multi-overlaps do not play any role in that case. Most of the rigorous results in the literature are concerned with such dense systems, one reason being that they are easier to study but still present a very rich phenomenology. As a consequence many concentration results are rigorously known for $Q_2$. In contrast, to the best of our knowledge, concentration results for {\it multi}-overlaps $Q_{k\ge3}$ as strong as Theorem \ref{prop:conc_overlap} were not present in the literature until now and we thus believe that it can be of independent interest. Note that the rigorous concentration results found in \cite{barra2007stability,sollich2012spin,barra2006overlap} are of a different nature than Theorem \ref{prop:conc_overlap}: In these references are proven so-called Aizenman-Contucci types of relations, that are hard contraints verified by the multi-overlap but that do {\it not} imply any concentration. Actually such relations, when they are verified, happen to be true independently of the fact that the multi-overlaps concentrate or not. The same is true for the so-called Ghirlanda-Guerra identities in spin glasses \cite{ghirlanda1998general}: These fundamental relations, which are linked to the ultra-metric structure of the overlaps, are valid even when the system has a ``glassy behavior'' where the overlaps are known not to concentrate as replica-symmetry breaking occurs.}\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we use this theorem to simplify the expression \eqref{eq:interpolation:main2} and \eqref{eq:interpolation:remainder} of the remainder. We have 
%
\begin{align}\label{decompo}
\sR_{t,s; h_0, \alpha}
= 
\widehat \sR_{t,s; h_0, \alpha} 
+
\mathcal{F}_{t,s; h_0, \alpha}
\end{align}
%
where
\begin{align}\label{Rhat}
 \widehat \sR_{t,s; h_0, \alpha} = \sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} \ \mathbb{E}  
\Big\langle (\tanh \tJ)^{k} \big(\mathbb{E}[\langle Q_{k}\rangle_{t,s; h_0, \alpha}]^p  - q_k^{(t) p}\big) - p \,\tilde{q}_k^{(t)} \big(\mathbb{E}[\langle Q_k\rangle_{t,s; h_0, \alpha}]  - q_k^{(t)} \big)
\end{align}
% 
and 
\begin{align}\label{F}
 \mathcal{F}_{t,s; h_0, \alpha} = \sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} (\tanh \tJ)^k \mathbb{E}\langle Q_k^p - \mathbb{E}[\langle Q_k\rangle_{t,s; h_0, \alpha}]^p\rangle_{t,s; h_0, \alpha}\,.
\end{align}
%
In Theorem \ref{prop:conc_overlap} the bound is uniform with respect to $s\in [0,1]$, $T$, and $t\in \{1, \cdots, T\}$. Therefore for any sequence $T_n$ such that $\lim_{n\to +\infty} T_n = +\infty$ we deduce for $M >1$ an arbitrary integer
%
\begin{align}
\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0 \biggl\vert \frac{1}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds\, \mathcal{F}_{t,s; h_0, \alpha}\biggr\vert 
\leq 
\frac{C(p, J)}{n^{1/12}} \sum_{k=1}^{M-1} \frac{(\tanh J)^k}{(\tanh h_1)^{k/2}} + \frac{2(\tanh J)^M}{M(1- \tanh J)}\,.
\end{align}
for any $0 <\underline h < \bar h < 1$, $0 < \underline \alpha <\bar \alpha<1$. Taking the limit $n\to +\infty$ (for fixed $M$) and $M\to +\infty$ afterwards we find
%
\begin{align}
\lim_{n\to +\infty}\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0 \biggl\vert \frac{1}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds\, \mathcal{F}_{t,s; h_0, \alpha}\biggr\vert = 0\, .
\end{align}
%
An elementary analysis argument (see Appendix \ref{elementaryapp}) then shows that one can find sequences
 $h_0^{(n)}, \alpha_0^{(n)} \to 0$ when $n\to +\infty$, such that 
%
\begin{align}\label{fluctzero}
 \lim_{n\to +\infty}\frac{1}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds\, \mathcal{F}_{t,s; h_0^{(n)}, \alpha^{(n)}} = 0\, .
\end{align}
%
Combining \eqref{eq:interpolation:main2}, \eqref{decompo}, \eqref{fluctzero} and Lemma \ref{proof:connection1} we arrive at
%
\begin{align}\label{first-simplif}
p_n  = {p}_{T_n}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0) + \frac{\gamma}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds \ \widehat \sR_{t,s; h_0^{(n)}, \alpha^{(n)}} + \smallO_n(1)
\end{align}

%
% Let $k_n\in \mathbb{N}^*$ such that $k_n\to +\infty$ as $n\to +\infty$. The rate of divergence will be adjusted later on. 
% We break the sum \eqref{eq:interpolation:remainder} in two parts
% \begin{align}
%  \sR_{t,s; h_0^{(n)}, \alpha^{(n)}} = \sR_{t,s; h_0^{(n)}, \alpha^{(n)}}^{(1)} +  \sR_{t,s; h_0^{(n)}, \alpha^{(n)}}^{(2)}
% \end{align}
% where the first term is the sum over $1\leq k\leq k_n$ and the second is the sum over $k\geq k_n$. Since 
% $\vert Q_k\vert \leq 1$, $\vert q_k\vert \leq 1$ and 
% $\vert\tilde{q}_k\vert \le (\tanh J)^k$ it is clear that 
% \begin{align}
%  \sR_{t,s; h_0^{(n)}, \alpha^{(n)}}^{(2)} \leq C_2\, p (\tanh J)^{k_n}
% \end{align}
% for some numerical constant $C_2 >0$. For the terms $1\leq k\leq k_n$ we will use 
% \begin{align}\label{concmultiover2}
% \int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0\,\frac{1}{T}\sum_{t=1}^T \int_0^1\,ds\,
% \mathbb{E} \big\< \big| Q_k^p - \mathbb{E}[\<Q_k\>_{t,s; h_0, \alpha}]^p \big| \big\>_{t,s; h_0, \alpha} \leq \frac{C_p k_n^{1/2}}{n^u}
% \end{align}
% which holds because the bound \eqref{concmultiover} is uniform in $T$ and $s\in [0,1]$.
% % 
% %
% \begin{align}
% {\cal R}_{t,s;h_0,\alpha}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}}) \equiv \sum_{k=1}^{k_{\rm max}}\frac{(-1)^{k+1}}{k} \ \mathbb{E}  \Big\langle (\tanh \tJ)^{k} \big(Q_{k}^{p} - (q_k^{(t)})^p\big) - p \,\tilde{q}_k^{(t)} \big(Q_k - q_k^{(t)} \big) \Big\rangle_{t,s; h_0, \alpha}\,.
% \end{align}
% %
% Each terms $\E\<-\>$ in this sum is bounded uniformly in $k$, $t$ and $s$ and thus Theorem \ref{prop:conc_overlap} implies directly
% %
% \begin{align}
% &\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0 \Big|\frac{1}{T}\sum_{t=1}^T\int_0^1ds\Big\{{\cal R}_{t,s;h_0,\alpha}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}})- {\cal R}_{t,s;h_0,\alpha}^{(k_{\rm max})}(\{\E\<Q_{k}\>_{t,s; h_0, \alpha}\}_{k=1}^{k_{\rm max}})\Big\} \Big| =  {\cal O}(n^{-u}k_{\rm max}^{3/2})\,.\label{28}
% \end{align}
% Now choose, say, $k_{\rm max}=\Theta(\ln n)$ (many other choices are fine, as long as $n^{-u}k_{\rm max}^{3/2}\to0$ and $k_{\rm max}\to\infty$ when $n\to\infty$; the requirement that $k_{\rm max}\to\infty$ will become clear very soon). With this choice, we can assert from \eqref{28} and using Lemma \ref{elementaryapp} twice that there exists a sequence $h_n\to 0_+$ and a sub-sequence $\alpha_n=\alpha_{h_n}\to\alpha$ for any $\alpha >0$, both independent of $t$ and $s$, such that 
% %
% \begin{align}
% \lim_{n\to\infty} \Big|\frac{1}{T}\sum_{t=1}^T\int_0^1ds\Big\{ {\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}}) - {\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{\E\<Q_{k}\>_{t,s; h_n, \alpha_n}\}_{k=1}^{k_{\rm max}})\Big\} \Big| = 0\,.	\label{conc_trunc_rema}
% \end{align}
% %
% Note that for using Lemma \ref{elementaryapp} we need to make sure that the integrand is continuous. It is not difficult to show the following general fact for well-defined statistical mechanics models: For any finite $n$ the free entropy, and thus the overlaps that are related to its derivatives, are analytic; phase transitions, i.e. non-analyticity points in the free entropy where the overlaps might jump in the case of first-order transitions, can only occur in the thermodynamic limit so we are safe.  We choose these particular sequences $h_n\to0_+$, $\alpha_n\to\alpha$. Again, each terms $\E\<-\>$ in the remainder \eqref{eq:interpolation:remainder} is bounded uniformly in $n$, $t$ and $s$. The full remainder can thus be written as
% %
% \begin{align}
% {\cal R}_{t,s;h_n,\alpha_n}(\{Q_{k}\}_{k\ge1})	={\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}}) + {\cal O}\Big(\sum_{k=k_{\rm max}+1}^\infty \frac{(\tanh J)^k + \tilde{q}_k^{(t)}}{k} \Big)\,.\label{30}
% \end{align}
% %
% Note that as $U^{(t)}\sim \tilde{\sfx}^{(t)}\in \tilde{{\cal P}}$ then by definition of $\tilde{{\cal P}}$ as being the set of distributions supported on $[0,J]$ with $J>0$ fixed and of $\tilde{q}_k^{(t)}\equiv\E[(\tanh U^{(t)})^k]$, we can assert that the ${\cal O}(\cdot)$ in the last identity is a convergent sum.
% % \begin{align}
% % \sum_{k=k_{\rm max}+1}^{\infty}\frac{\tilde{q}_k^{(t)}}{k} ={\cal O}\Big(\sum_{k= k_{\rm max}+1}^\infty \frac{1}{k^{1+\epsilon}}\Big)
% % \end{align}
% % for some $\epsilon >0$ and is thus a convergent sum. 
% Recalling that $k_{\rm max}$ diverges with $n$ this sum converges to $0$ (this is the reason of the requirement that $k_{\rm max}$ is an increasing sequence with $n$) and thus the overall ${\cal O}(\cdot)$ in \eqref{30} is a $\smallO_n(1)$, where all along this paper we denote $\smallO_n(1)$ a quantity such that $\lim_{n\to\infty}\smallO_n(1)=0$ independently of everything else. The identity \eqref{30}, when combined with \eqref{conc_trunc_rema}, then implies that
% %
% \begin{align}
% &\frac{1}{T}\sum_{t=1}^T\int_0^1ds\,{\cal R}_{t,s;h_n,\alpha_n}(\{Q_{k}\}_{k\ge1})	\nonumber\\
% = &\ \frac{1}{T}\sum_{t=1}^T\int_0^1ds\,{\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{\E\<Q_{k}\>_{t,s; h_n, \alpha_n}\}_{k=1}^{k_{\rm max}}) + \smallO_n(1)\nonumber\\
% %
% = &\ \frac{1}{T}\sum_{t=1}^T\int_0^1ds\,\sum_{k=1}^{k_{\rm max}} \frac{(-1)^{k+1}}{k} \Big \{ (\tanh \tJ)^{k} \big( \mathbb{E}[ \< Q_{k} \>_{t,s; h_n, \alpha_n} ]^{p} - (q_k^{(t)})^p \big) \nonumber\\
% &\hspace{5cm}- p\, \tilde{q}_k^{(t)} \big( \mathbb{E} \< Q_k \>_{t,s;h_n, \alpha_n}  - q_k^{(t)} \big) \Big \} + \smallO_n(1) \,.\label{eq:interpolation:remainder:concentrated1}
%\end{align}
%

We will further simplify \eqref{first-simplif} thanks to the following crucial lemma:
%
\begin{lemma}[Weak $s$-dependence at fixed $t$]\label{lemma:weakdep}
For any $s \in [0,1]$ we have
%
\begin{align}
\big| \mathbb{E} \< Q_k \>_{t,s; h_0, \alpha_0} - \mathbb{E} \< Q_k \>_{t,0; h_0, \alpha_0} | \leq  \frac{(4p+1)\gamma n k}{T}\,.
\end{align}
%
the same inequality holds with $h_0$, $\alpha$, $T$ replaced by sequences $h_0^{(n)}$, $\alpha^{(n)}$, $T_n$.
\end{lemma}
%
\begin{proof}
The proof is immediate using an interpolation. Using the property \eqref{eq:dPoissonMean} in Appendix \ref{poisson-appendix} of Poisson distributions we find
\begin{align}
&\mathbb{E} \< Q_k \>_{t,s; h_0^{(n)}, \alpha^{(n)}}   -  \mathbb{E}\< Q_k \>_{t,0; h_0^{(n)}, \alpha^{(n)}} 
	 = \frac{1}{n} \int_{0}^{s} ds' \sum_{i=1}^{n} \frac{d}{ds'} \mathbb{E}  \< \sigma_i \>_{t,s'; {h}_n, \alpha_n}^k  \nonumber \\
	&\qquad \qquad = \frac{1}{n} \int_{0}^{s} ds' \sum_{i=1}^{n} \mathbb{E} \Big [ \frac{\gamma pk}{T} \sum_{j=1}^{n} \Big ( \< \sigma_i \>_{e_{j,s'}^{(t)} + 1}^{k-1} 
	- \< \sigma_i \>_{e_{j,s'}^{(t)}}^{k-1} \Big) - \frac{\gamma nk}{T} \Big ( \< \sigma_i \>_{m_{s'}^{(t)} + 1}^{k-1} - \< \sigma_i \>_{m_{s'}^{(t)}}^{k-1} \Big ) \Big] \,.
	\nonumber
\end{align}
From $| \< \sigma_i \> |\le 1$ we easily obtain the result. The same proof is valid with $h_0$, $\alpha$, $T$ replaced by sequences $h_0^{(n)}$, $\alpha^{(n)}$, $T_n$.
\end{proof}
%

Note that $T$ is a {\it free} parameter controlling the mean of $e_{i,s}^{(t)}$ and $m_s^{(t)}$ and can thus be set arbitrarily large. Thus we choose $T_n$ such that $n/T_n = \smallO_n(1)$. Using Lemma \ref{lemma:weakdep},  \eqref{Rhat} 
(and $\vert Q_k\vert \leq 1$, $\vert q_k\vert \leq 1$, $\vert\tilde{q}_k\vert \le (\tanh J)^k$) 
we can simplify \eqref{first-simplif} to finally obtain
%
\begin{align}\label{second-simplif}
p_n  = {p}_{T_n}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0) + \frac{\gamma}{T_n} \sum_{t=1}^{T_n}\widehat \sR_{t,0; h_0^{(n)}, \alpha^{(n)}} + \smallO_n(1)
\end{align}
%
where the remainder now takes the form
%
\begin{align}\label{Rhat-s=0}
 \widehat \sR_{t,0; h_0^{(n)}, \alpha^{(n)}} = \sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} \biggl\{ 
(\tanh \tJ)^{k} \big(\mathbb{E}[\langle Q_{k}\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}]^p  - q_k^{(t) p}\big) - p \,\tilde{q}_k^{(t)} \big(\mathbb{E}[\langle Q_k\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}]  - q_k^{(t)} \big)\biggr\}
\end{align}
%
Equations \eqref{second-simplif} and \eqref{Rhat-s=0} form the basis for the upper and lower bounds of the next section.

%Therefore thanks to 
%Lemma~\ref{lemma:weakdep} and choosing $T\gg n k_{\rm max}$, we can remove the dependence of $\sR_{t,s; h_n, \alpha_n}$ on $s$ by re-writing \eqref{eq:interpolation:remainder:concentrated1} as
%%
%\begin{align}
%&\qquad \qquad \frac{1}{T}\sum_{t=1}^T\int_0^1ds\,{\cal R}_{t,s;h_n,\alpha_n}(\{Q_{k}\}_{k\ge1})\label{eq:interpolation:remainder:concentrated2}\\
%=& \ \frac{1}{T}\sum_{t=1}^T\sum_{k=1}^{k_{\rm max}} \frac{(-1)^{k+1}}{k} \Big \{ (\tanh \tJ)^{k} \big( \mathbb{E}[ \< Q_{k} \>_{t,0; h_n, \alpha_n} ]^{p} - (q_k^{(t)})^p \big) - p\, \tilde{q}_k^{(t)} \big( \mathbb{E} \< Q_k \>_{t,0;h_n, \alpha_n}  - q_k^{(t)} \big) \Big \} + \smallO_n(1)\,.\nonumber
%\end{align}
%%
%Lemma~\ref{thm:bd_fixed_t} is critical because $\mathbb{E}\langle Q_{p} \rangle_{t,s=0; {h}_n, \alpha_n}$ is independent of $\{ \sfx^{(t')},\tilde{\sfx}^{(t')} \}_{t' \geq t}$ an in particular of $\sfx^{(t)}$, $\tilde{\sfx}^{(t)}$ (this is only true at $s=0$ thus this specific choice). This allows an {\it adaptive} choice of \ $\tilde{\sfx}^{(t)}$ and $\sfx^{(t)}$ from $t=1$ to $T$, thus the name of the method, eventually leading to the following bounds by canceling term by term the remainder along the interpolation path.
%%%%%


==> sections/concentrationtheorems.tex <==
\section{Concentration of Multioverlaps}\label{concentrationtheorems}

The {\it multioverlaps} are defined for any integer $k\geq 1$ as 
\begin{align}
 Q_k = \frac{1}{n}\sum_{i=1}^n \sigma_i^{(1)}\cdots \sigma^{(k)}
\end{align}
where $\{\bsig^{(\alpha)}, \alpha=1, \cdots, k\}$ is a set of $k$ {\it replicas} of the spin configurations drawn according to the $k$-fold tensor product of the Gibbs measure. We emphasize that 
In this work
the replicas are always uncoupled and iid. The Gibbs average with respect to the tensor product Gibbs measure is still indicated as $\langle - \rangle$. The whole set of ``order parameters'' 
\begin{align}
 \langle Q_k\rangle = \frac{1}{n}\sum_{i=1}^n \langle \sigma_i^{(1)}\cdots \sigma^{(k)}\rangle = \frac{1}{n}\sum_{i=1}^n \langle \sigma_i\rangle^k, \quad k\geq 1
\end{align}
plays a fundamental role in the solution of the model. 

Among our main results are concentration theorems for the multioverlaps. This requires the introduction of small perturbations, which are introduced later on, 
whose role is to select ``pure states.'' With suitable such perturbations we show that: (i) for any instance of the random graph $Q_k$ concentrates over $\langle Q_k\rangle$; (ii) and 
$\langle Q_k\rangle$ concentrates over $\mathbb{E}\langle Q_k\rangle$. These two concentration properties imply that overall $Q_k$ concentrates on $\mathbb{E}\langle Q_k\rangle$. 
According to the replica/cavity theories
concentration of the overlaps implies that the pressure is given by the replica symmetric formula. As an application of the concentration properties we can prove a one sided 
bound supporting this conjecture. The proof proceeds via a formulation of the recently developped adaptive interpolation method for the Erdoes-R\'enyi graph. We 
believe that various other results obtained along the way are important stepping stones for a complete proof of the replica formula. 
The precise formulation and possible extensions of these results beyond the ferromagnetic case are discussed at more length in Section \ref{mainresults}.

Our analysis of the concentration properties applies to any ``reasonable'' dilute ferromagnetic random spin model for which the pressure concentrates 
in a second moment sense. For example the random graph ensemble can be Erd\"os-R\'enyi, it can be the set of $d$-regular graphs, or more geenrally, in the factor graph language we can take a 
$(\Lambda, P)$ ensemble (see \ref{} for exact definitions). Once the concentration of the pressure is estabished the ensemble does not play an important role in the analysis so we choose not to 
discuss all ensembles in detail and we restict ourselves to the essential aspects. 

We consider 
a generic ferromagnetic system of the form \eqref{mostgeneralhamiltonian} to which we add a perturbation 
term $\sH_{\mathrm{pert}}(\bsig)$ of the form
\begin{align}
\sH_{\mathrm{pert}}(\bsig) \equiv - h_0 \sum_{i=1}^{n} \sigma_i - h_1 \sum_{i=1}^n \tau_i \sigma_i\label{pert}
\end{align}
with $h_0, h_1\in [0,1]$, $\tau_i \sim \mathrm{Poi}(\alpha n^{\theta-1})$ iid for $i=1,\ldots,n$ and $\alpha\in [0,1]$, $\theta \in \big (1/2, 5/6)$.
The first part of the perturbation, proportional to $h_0$, is called {\it homogeneous perturbation} while the second part proportional to $h_1$ is called
{\it Poisson perturbation}. Both are purely ferromagnetic such that the GKS inequalities remain valid. Note that in 
distribution $h_1 \sum_{i=1}^n \tau_i \sigma_i \stackrel{d}{=} h_1 \sum_{v=1}^{\Gamma} \sigma_{i_v}$
where $\Gamma \sim \mathrm{Poi}(\alpha n^{\theta})$ and $i_v$ is randomly and uniformly chosen from $\{1,\dots,n\}$.
While this second expression might seem more natural, the first equivalent expression allows a more compact notation in our analysis.

We associate to the Hamiltonian \eqref{pert_H} its 
partition function ${\cal Z}_{h_0, h_1, \alpha}$, Gibbs expectation $\<-\>_{h_0, h_1, \alpha}$, pressure $P_n(h_0, h_1, \alpha)= n^{-1}\ln {\cal Z_{h_0, h_1, \alpha}}$ and average pressure 
$p_n(h_0, h_1, \alpha) = \mathbb{E}P_n(h_0, h_1, \alpha)$. Here $\mathbb{E}$ is the expectation over all quenched variables
i.e., $J_X$, $X\subset\{1, \cdots, n\}$ and $\btau = (\tau_1, \cdots, \tau_n)$.
For all this section we do not indicate explicitly the dependencies in the perturbation 
parameters $h_0$, $\alpha$ for the sake of readibility.
We suppose that the pressure associated to \eqref{pert_H} concentrates, namely that there exists a constant $C>0$ such that 
\begin{align}\label{concpressuregeneral}
 \mathbb{E}[(P_n(h_0, h_1, \alpha) - p_n(h_0, h_1, \alpha)^2] \leq \frac{C}{n}
\end{align}
Because $h_0, h_1, \alpha\in (0,1)$ the constant $C$ can be made independent of these parameters. 
In appendix \ref{sec:free_ent_conc} it is shown by standard methods that this is valid for the $p$ spin model \ref{eq:Gibbs} (with the added perturbation) on 
the Erd\"os-R\'enyi ensemble and that the constant $C$ depends only on $p$ and $J$.

Finally an elementary argument shows that the perturbation does not modify the thermodynamic properties as long as $h_0 \to 0$ ($\alpha$ can be taken fixed). In Appendix \ref{elementaryapp} we show
\begin{align}
 \vert p_n(h_0, h_1, \alpha) - p_n(0,0,0) \vert \leq h_0 + \frac{h_1}{n^{1-\theta}} 
\end{align}

We can now state the main concentration results
%
%%%% -- thermal concentration --
\begin{theorem}[Thermal concentration]
Assume $\sH(\bsig)$ in \eqref{pert_H} satisfies $\< \sigma_i \sigma_j \> - \< \sigma_i \> \< \sigma_j \> \geq 0$ for all $i, j=1, \cdots, n$. 
Then for any $[\underline{h}, \bar h]\subset (0,1)$, $h_1, \alpha\in [0,1]$, we have for any instance of the random Hamiltonian
\begin{align}
\int_{\underline{h}}^{\bar h} dh_0 \,\big\< \big(Q_k - \< Q_k \>_{h_0, h_1, \alpha}\big)^2 \big\>_{h_0, h_1, \alpha}
	\leq \frac{2k}{n}\,.
\end{align}
\end{theorem}
%

\begin{theorem}[Total concentration of the magnetization/first overlap]
Assume $\sH(\bsig)$ in \eqref{pert_H} satisfies $\< \sigma_i \sigma_j \> - \< \sigma_i \> \< \sigma_j \> \geq 0$ for all $i, j=1, \cdots, n$ and assume also that 
the pressure concentrates as in \eqref{concpressuregeneral}.
Then for any $[\underline{h},\bar h]\subset (0,1)$, $h_1, \alpha\in [0,1]$ we have
\begin{align}
\int_{\underline{h}}^{\bar h} dh_0 \,\mathbb{E}\big\< \big(Q_1 - \mathbb{E}\< Q_1 \>_{h_0, h_1, \alpha}\big)^2 \big\>_{h_0, h_1, \alpha}
	\leq \frac{C}{n^{1/3}}\,.
\end{align}
\end{theorem}
% 

Let us make a few remarks about these two theorems. First of all the Poisson perturbation is not needed and we can set $h_1=\alpha=0$. More importantly, 
Assuming only $\< \sigma_i \sigma_j \> - \< \sigma_i \> \< \sigma_j \> \geq 0$ is weaker than assuming both GKS inequalities and even weaker than assuming 
only the second one. This assumption is satisfied (for example) for all Hamiltonians 
satisfying the FKG inequality. An example is $J_X\geq 0$ except for one-body terms (magnetic fields) that may have any sign. Another example is strong enough ferromagnetic two-body terms and any sign for 
magnetic fields and higher order interactions. This remark is not used explicitly in the pesent work but we believe it could be useful for the RFIM. 
%

The next theorem assumes both GKS inequalities and the extension to systems satisfying only FKG is an open problem. Moreover both teh homogeneous and teh Poisson perturbation play an important role in the proof. 

\begin{theorem}[Multioverlap concentration]
Assume $\sH(\bsig)$ in \eqref{pert_H} satisfies both GKS inequalities and also that the free entropy concentrates as in 
\eqref{concpressuregeneral}. Then for any $[\underline h, \bar h]\subset (0,1)$, $[\underline\alpha, \bar\alpha]\subset (0,1)$, $h_1\in (0,1]$, $\theta \in  ( 1/2, 5/6 )$  we have
\begin{align}
\int_{\underline h}^{\bar h} dh_0 \int_{\underline \alpha}^{\bar \alpha} d\alpha \, 
\mathbb{E}\big\< \big(Q_k - \mathbb{E} \< Q_k \>_{h_0, h_1, \alpha} \big)^2\big\>_{h_0, h_1, \alpha}
\leq\frac{3 k^2}{(\tanh h_1)^{k}} \frac{(5C + 160)^{1/2}}{n^{1/6}} \,.
\end{align}
\end{theorem}

Note that the prefactor on teh r.h.s grows exponentially fast with $k$. We can make this dependence into a $)(k^2)$ by taking $h_1= O(\ln n)$. The details of the proof
show that a slowly growing $h_1$ can be accomodated. 

These three theorems are proven in Section \ref{sec:conc}.



==> sections/interpolation.tex <==
\section{Adaptive path interpolation method}\label{interpolation}

In this section we develop the adaptive interpolation method for the $p$-spin dilute ferromagnetic 
model of example \ref{ex1}. Our basic result are equations \eqref{second-simplif}, \eqref{Rhat-s=0} at the end of this section. These relations form the 
basis for proving Proposition \ref{bound2} in Section \ref{cancelling}.

\subsection{The $(t,s)$--interpolating model}\label{sec:sparse:Kint:int-model}
%
We construct a $p$-spin model which interpolates between the $p$-spin model 
\eqref{eq:Gibbs} and a "mean field" model of independent spins in effective magnetic fileds. 
The interpolation involves both discrete and continuous time parameters $t \in \{1, 2, \ldots, T \}$ where $T$ is a (large) integer and $s \in [0,1]$. 
The discrete index $t$ represents a {\it global} interpolation parameter, while the continuous time $s$ serves a {\it local} 
interpolation between successive discrete time steps.
The precise construction of an interpolating ensemble $\sG_{t,s}$ for $t \in \{1, 2, \ldots, T \}$ and $s \in [0,1]$ is given in  Algorithm 1. 
The interpolated graph is designed such that $\sG_{t,1}$ is statistically equivalent to $\sG_{t+1,0}$; in addition, $\sG_{t,s}$ maintains 
the distribution of variable nodes degree invariant for different $t$ and $s$.
\begin{algorithm}
\caption{Construction of $\sG_{t,s}$}
\begin{algorithmic}
\label{algo:G(t,s)}
\For {$t' = 1, \dots, t-1$}
	\For {$i = 1, \dots, n$}
		\State {\_draw a random number $l_i^{(t')} \sim \mathrm{Poi}\big ( \frac{p}{RT} \big )$}
		\For {$b = 1, \dots, l_i^{(t')}$}
			\State{\_connect variable node $i$ with a half edge with weight $U_{b \rightarrow i}^{(t')} \sim \tilde{\sfx}^{(t')} \in \tilde{\mathcal{P}}$}
		\EndFor
	\EndFor
\EndFor
%
\vspace{3pt}
\For {$t' = t+1, \dots, T$}
	\State {\_draw a random number $m^{(t')} \sim \mathrm{Poi}\big ( \frac{n}{RT} \big )$}
	\For {$A^{(t')} = 1, \dots, m^{(t')}$}
		\State {\_associate factor node $A^{(t')}$ with weight $\tJ$}
		\State {\_connect node $A^{(t')}$ to $p$ variable nodes chosen uniformly at random (and the subset of the variable} 
		\hspace{1cm}\State{nodes is denoted by $A^{(t')}$)}
	\EndFor
\EndFor
%
\vspace{3pt}
\For {$i = 1, \dots, n$}
	\State {\_draw a random number $l_{i,s}^{(t)} \sim \mathrm{Poi}\big( \frac{ps}{RT} \big)$}
	\For {$b = 1, \dots, l_{i,s}^{(t)}$}
		\State{\_connect variable node $i$ with a half edge with weight $U_{b \rightarrow i}^{(t)} \sim \tilde{\sfx}^{(t)} \in \tilde{\mathcal{P}}$}
	\EndFor
\EndFor
%	
\vspace{3pt}
\State {\_draw a random number $m_s^{(t)} \sim \mathrm{Poi}\big( \frac{n(1-s)}{RT}\big)$}
\For {$A^{(t)} = 1, \dots, m_s^{(t)}$}
	\State {\_associate factor node $A^{(t)}$ with weight $\tJ$}
	\State {\_uniformly and randomly connect node $A^{(t)}$ to $p$ variable nodes}
\EndFor
%
\vspace{3pt}
\For {$i = 1, \dots, n$}
	\State{\_connect variable node $i$ with a half edge with weight $H$}
\EndFor
\end{algorithmic}
\end{algorithm}
The $p$-spin interpolating Hamiltonian associated with the graph ensemble $\sG_{t,s}$ is 
\begin{align}
\sH_{t,s}(\bsig, \bU, \textbf{m}, \textbf{l}) 
	= \-
	- \sum_{t'=1}^{t-1} \sum_{i=1}^{n} \sum_{b=1}^{l_{i}^{(t')}} U_{b \rightarrow i}^{(t')} \sigma_i 
	- \tJ \sum_{t' = t+1}^T \sum_{A^{(t')}=1}^{m^{(t')}} \sigma_{A^{(t')}} 
	- \sum_{i=1}^{n} \sum_{b=1}^{l_{i,s}^{(t)}} U_{b \rightarrow i}^{(t)} \sigma_i
	- \tJ \sum_{A^{(t)}=1}^{m_s^{(t)}} \sigma_{A^{(t)}}
	- H \sum_{i=1}^{n} \sigma_i\,.
\label{eq:Hamiltonian_ts}
\end{align}
%
We will need a further generalized version of \eqref{eq:Hamiltonian_ts} involving two external magnetic field perturbations.
Thus our final interpolating Hamiltonian is
\begin{align}
\sH_{t,s; h_0,\alpha}(\bsig, \bU, \textbf{m}, \textbf{l}, \boldsymbol{\tau}) 
	& = \sH_{t,s}(\bsig, \bU, \textbf{m}, \textbf{l}) - h_0 \sum_{i=1}^{n} \sigma_i - h_1 \sum_{i = 1}^{n} \tau_i \sigma_i\,.
	\label{eq:Hamiltonian_tse}
\end{align}
%
where $h_0 \geq 0$, $h_1\ge 0$ and $\tau_i \sim \mathrm{Poi}(\alpha n^{\theta-1})$, $\theta\in(1/2,1)$. 
Later on we call the first perturbation (proportional to $h_0$) the {\it homogeneous perturbation} while the 
second one (proportional to $h_1$) is the {\it Poisson perturbation}. 
It is important that both are purely ferromagnetic, i.e. $h_0,h_1\geq 0$. 
The associated Gibbs expectation and pressure are
\begin{align}
% {\cal Z}_{t,s; h_0,\alpha}
% 	& \equiv \sum_{\bsig\in\{\pm1\}^n} \exp(-\sH_{t,s; h_0,\alpha}(\bsig, \bU, \textbf{m}, \textbf{l}, \boldsymbol{\tau}) ) \label{eq:partitionFunction_tse}\,, \\
\< \sigma_R \>_{t,s; h_0,\alpha} 
	& = \frac{1}{{\cal Z}_{t,s;h_0,\alpha}}\sum_{\bsig\in\{\pm1\}^n} \sigma_R \exp(-\sH_{t,s; h_0,\alpha}(\bsig, \bU, \textbf{m}, \textbf{l}, \boldsymbol{\tau}))\,, \label{eq:GibbsExp_tse} \\
P_{n, t,s}(h_0,\alpha) & = \frac{1}{n} \ln {\cal Z}_{t,s;h_0,\alpha}\,, \label{11}\\
p_{n, t,s}(h_0,\alpha) & = \mathbb{E} P_{n, t,s}( h_0,\alpha) \,.\label{12}
\end{align}
%
Again, we write $\mathbb{E}$ to denote an expectation over all (quenched) random variables appearing 
in the interpolating model. 
% Note that ${\cal Z}_{t,s; h_0,\alpha}$, ${P}_{t,s; h_0,\alpha}$ and 
% Gibbs-Boltzmann expectations $\langle - \rangle_{t,s; h_0,\alpha}$ as well are 
% functions of all the quenched random variables (i.e. of ${\cal G}_{t,s}$). The same remark applies for the $n$-dependence. 
The interpolating model is purely ferromagnetic (i.e., with positive coupling constants and fields) so that the GKS inequalities are valid for the bracket
$\langle - \rangle_{t,s; h_0, \alpha}$
\begin{align}
& \< \sigma_S \>_{t,s; h_0, \alpha} \geq 0\,, \label{eq:GKS1} \\
& \< \sigma_S \sigma_T \>_{t,s; h_0, \alpha} - \< \sigma_S \>_{t,s; h_0, \alpha} \< \sigma_T \>_{t,s; h_0, \alpha} \geq 0\,. \label{eq:GKS2}
\end{align}

The connection between the unperturbed and perturbed 
interpolating free entropies  is given by the following simple lemma proven in Appendix~\ref{proof3.3}
%
\begin{lemma}\label{proof:connection1}
For any sequence $h_0^{(n)} \rightarrow 0_{+}$ and $\alpha^{(n)}\to\alpha \geq 0$ we have
\begin{align*}
\lim_{n \rightarrow \infty} \big|p_{n,t,s}(h_0^{(n)}, \alpha^{(n)}) - p_{n,t,s}(0,\alpha)\big| = 0\,.
\end{align*}
where the limit is uniform in $s\in [0,1]$, $t=1,\dots, T$. 
\label{thm:connection1}
\end{lemma}
%

%%%%
\subsection{Fundamental sum rule}
%
Recall that ${\cal G}_{t,1}$ is statistically equivalent to ${\cal G}_{t+1,0}$ and thus $f_{t,1; h_0,\alpha}=f_{t+1,0; h_0,\alpha}$ for all $t=1,\ldots, T-1$. 
By interpolating $p_{n, t,s}( h_0, \alpha)$ from the initial state $(t=1, s=0)$ to the final one $(t=T, s=1)$ and using this invariance property, we have the following identity:
\begin{align}
p_{n, 1,0}(h_0, \alpha) & = p_{n,T,1}( h_0, \alpha) + \sum_{t=1}^{T} ( p_{n, t,0} (h_0, \alpha) - p_{n, t,1} (h_0, \alpha)) 
\nonumber \\ &
= p_{n, T,1} (h_0, \alpha) - \sum_{t=1}^T \int_0^1 ds \frac{dp_{n, t,s} (h_0, \alpha)}{ds}\,.
\label{eq:interpolation:main1}
\end{align}
Let us first discuss the two  boundary terms $p_{n, 1,0}(h_0, \alpha)$ and $p_{n, T,1} (h_0, \alpha)$.
It is easy to see 
starting from \eqref{eq:Hamiltonian_ts}, \eqref{eq:Hamiltonian_tse} that, due to 
the fact that a sum of independent Poisson-distributed random variables is also Poisson distributed, one has the following equalities in distribution:
\begin{align*}
\sH_{1,0; h_0, \alpha} 
	& = - \tJ \sum_{t=1}^{T} \sum_{A^{(t)}=1}^{m^{(t)}}  \sigma_{A^{(t)}} - H\sum_{i=1}^{n} \sigma_i - h_0 \sum_{i=1}^{n} \sigma_i - h_1 \sum_{i = 1}^{n} \tau_i \sigma_i \nonumber\\
	&\stackrel{d}{=} - \tJ\sum_{A=1}^{m}  \sigma_{A} - H\sum_{i=1}^{n}  \sigma_i - h_0 \sum_{i=1}^{n} \sigma_i - h_1 \sum_{i = 1}^{n} \tau_i \sigma_i\,.
\end{align*}
Therefore the initial value of the interpolating free entropy - when no perturbation is taken into account - is nothing but simply the free entropy \eqref{freeentpspin}: 
$p_{n, 1,0}( 0, 0)=p_n$. Since we need later on to use the perturbation terms we will write 
%
\begin{align}\label{20}
p_{n, 1,0}(h_0, \alpha) = p_n + ( p_{n, 1,0}(h_0, \alpha) - p_{n, 1,0}(0, 0) )\,. 
\end{align}
where the term $p_{n, 1,0}(h_0, \alpha) - p_{n, 1,0}(0, 0)$ tends to zero along any sequence $h_0^{(n)}, \alpha^{(n)} \to 0$ (because of Lemma \ref{proof:connection1}).
On the other hand, $p_{T,1}( h_0, \alpha)$ corresponds to a part of the generalized functional \eqref{eq:RSFreeEntropy_coupled1}. Indeed
from \eqref{eq:Hamiltonian_ts} and \eqref{12} we find
\begin{align}
p_{n,T,1}( {h}_0, \alpha) 
	& = \frac{1}{n} \mathbb{E} \ln \sum_{{\bsig\in\{\pm1\}^n}} \exp \Big( \sum_{t=1}^{T} \sum_{i=1}^{n} \sum_{b=1}^{l_{i}^{(t)}} U_{b \rightarrow i}^{(t)} \sigma_i + H \sum_{i=1}^{n} \sigma_i + {h}_0 \sum_{i=1}^{n} \sigma_i + {h}_1 \sum_{i = 1}^{n} \tau_i \sigma_i \Big ) \nonumber \\
	& = \frac{1}{n}\sum_{i=1}^n \mathbb{E} \ln \sum_{\sigma_i = \pm 1} \exp \Big(\sigma_i \Big\{\sum_{t=1}^{T} \sum_{b=1}^{l_{i}^{(t)}} U_{b \rightarrow i}^{(t)}  + H + {h}_0+{h}_1 \tau_i \Big\}\Big ) \nonumber \\
	& = \mathbb{E} \ln \Big ( e^{H + {h}_0 + {h}_1 \tau_1} \prod_{t=1}^{T} \prod_{b=1}^{l_{1}^{(t)}} (1 + \tanh U_{b}^{(t)}) + e^{-H - {h}_0 - {h}_1 \tau_1} \prod_{t=1}^{T} \prod_{b=1}^{l_{1}^{(t)}} (1 - \tanh U_{b}^{(t)}) \Big) \nonumber\\
	&\qquad \qquad + \frac{\gamma p}{T}\sum_{t=1}^{T} \mathbb{E} \ln \cosh U^{(t)} 	\label{eq:h_T1}
\end{align}
where the last line follows from $e^{\sigma x} = \cosh x (1 +\sigma \tanh x)$ for $\sigma=\pm1$. Comparing with \eqref{eq:RSFreeEntropy_coupled1} we find
\begin{align}
 p_{n, 1,0}(h_0, \alpha)  =  & {p}_{T}( \underline{\sfx}, \underline{\tilde{\sfx}}; h_0, \alpha ) + \frac{\gamma p}{T}\sum_{t=1}^{T} \mathbb{E} \ln \cosh U^{(t)} 
 - \frac{\gamma}{T} \sum_{t=1}^{T} \E\ln \Big( 1 + \tanh \tJ \prod_{i=1}^{p} \tanh V_i^{(t)} \Big) 
 \nonumber \\ &
	 + \frac{\gamma p}{T} \sum_{t=1}^{T}\E \ln \Big( 1 + \tanh U^{(t)} \tanh V^{(t)} \Big)  - \gamma \ln \cosh \tJ\,.
	 \label{boundary2}
\end{align}
%
Therefore replacing \eqref{20}, \eqref{boundary2} in \eqref{eq:interpolation:main1} for any sequence $h_0^{(n)}, \alpha^{(n)} \to 0$ and using Lemmas \ref{proof:connection1}, \ref{smallnesspertfunct} in Appendix \ref{proof3.3} we obtain 
\begin{align}
 p_n = & \, {p}_{T}( \underline{\sfx}, \underline{\tilde{\sfx}}; 0, 0) - \sum_{t=1}^T \int_0^1 ds \frac{dp_{n, t,s} (h_0, \alpha)}{ds}
 \nonumber 
 \\ &
 + \frac{\gamma p}{T}\sum_{t=1}^{T} \mathbb{E} \ln \cosh U^{(t)} 
 - \frac{\gamma}{T} \sum_{t=1}^{T} \E\ln \Big( 1 + \tanh \tJ \prod_{i=1}^{p} \tanh V_i^{(t)} \Big) 
 \nonumber \\ &
+ \frac{\gamma p}{T} \sum_{t=1}^{T}\E \ln \Big( 1 + \tanh U^{(t)} \tanh V^{(t)} \Big)  - \gamma \ln \cosh \tJ + \big( p_{n, 1,0}(h_0, \alpha) - p_{n, 1,0}(0, 0) \big)\, .
\label{sumR}
\end{align}
%where $\lim_{n\to +\infty}o_n(1) =0$ (from the bounds in Appendix \ref{proof3.3} this convergence is uniform with respect to $J$, $H$, $\gamma$, $T$, $\underline\sfx$, $\tilde{\underline\sfx}$).

The next step is to compute the $s$-derivative in the integral. 
Thanks to the Poisson property \eqref{eq:dPoissonMean} in Appendix \ref{poisson-appendix} we find
\begin{align}
\frac{dp_{t,s}({h}_0, \alpha)}{ds} \-
	& = - \frac{\gamma}{T} \mathbb{E}\,\mathbb{E}_{B} \ln \< e^{\tJ \sigma_{B}} \>_{t,s; {h}_0, \alpha} 
		+ \frac{\gamma p}{nT} \sum_{i=1}^{n} \mathbb{E}\,\mathbb{E}_{U_i^{(t)}} \ln \< e^{U_{i}^{(t)} \sigma_{i}} \>_{t,s; {h}_0, \alpha} \,.
		\label{eq:dh_ts}
\end{align}
Here the Gibbs expectation $\<-\>_{t,s; {h}_0, \alpha}$ defined by \eqref{eq:GibbsExp_tse} 
is performed under the original interpolating graph ensemble; thus 
the additional factors $J \sigma_B$ and $U_i^{(t)}\sigma_i$ do {\it not} enter in this bracket. Moreover we have separted explicitly the expectation $\mathbb{E}$ over quenched 
variables entering in the Gibbs bracket and the {\it new} quenched variables.
In the first term we emphasize this, by writing explicitely $\E_B$, which is an average over the random uniform selection of 
the spins entering the {\it new} product $\sigma_B=\sigma_{i_1}\dots\sigma_{i_p}$. 
Similarly for the second term we emphasize this by explicitly writing the expectation over a
{\it new} field $U_i^{(t)}\sim \tilde{\sfx}^{(t)}$. 
We now again apply the identity $e^{\pm x} = \cosh x (1 \pm \tanh x)$ followed by the Taylor expansion of the logarithm in order to obtain 
(for the end of the derivation we simply write $\<-\>$ 
instead of $\<-\>_{t,s; {h}_0, \alpha}$ and $\E$ for the expectation with respect to all quenched random variables entering the graph ensemble ${\cal G}_{t,s}$ {\it and} the newly added ones)
\begin{align*}
-\frac{\gamma}{RT}\mathbb{E} \,\mathbb{E}_B\ln \< e^{\tJ \sigma_{B}} \>_{t,s; {h}_0, \alpha} 
	& = -\frac{\gamma}{T}\mathbb{E}\, \mathbb{E}_B  \ln ( 1 + \langle \sigma_B \rangle_{t,s; {h}_0, \alpha}\tanh \tJ )  -\frac{\gamma}{T} \ln \cosh \tJ \nonumber \\
	& = -\frac{\gamma}{T}\sum_{k=1}^{\infty} \frac{(-1)^{k+1}}{k n^p}\sum_{i_1,\dots,i_p} \mathbb{E}  [\langle \sigma_{i_1} \cdots \sigma_{i_p} \rangle_{t,s; {h}_0, \alpha}^k]   
	( \tanh \tJ )^k -\frac{\gamma}{RT} \ln \cosh \tJ\,. 
\end{align*}
For the second term we obtain similarly
\begin{align*}
\frac{\gamma p}{nT} \sum_{i=1}^{n} \mathbb{E}\, \mathbb{E}_{U_{i}^{(t)}}\ln \< e^{U_{i}^{(t)} \sigma_{i}} \>_{t,s; {h}_0, \alpha}
	& = \frac{\gamma p}{nRT} \sum_{i=1}^{\infty} \mathbb{E}\,\mathbb{E}_{U_{i}^{(t)}}\ln( 1 + \langle \sigma_i \rangle_{t,s; {h}_0, \alpha} \tanh U_i^{(t)}  )  
	+ \frac{\gamma p}{T}\mathbb{E}\ln \cosh U^{(t)} \nonumber \\
	& = \frac{\gamma p}{T}\sum_{k=1}^{\infty} \frac{(-1)^{k+1}}{kn}  
	  \sum_{i=1}^n\mathbb{E}[\langle \sigma_i \rangle_{t,s; {h}_0, \alpha}^k]  \mathbb{E} [ (\tanh U^{(t)})^k ] + \frac{\gamma p}{T}\mathbb{E} \ln \cosh U^{(t)}\,.
\end{align*}

We now  define the moments
%
\begin{align}
q_k^{(t)} = \mathbb{E} [(\tanh V^{(t)})^k]\,,\qquad \tilde{q}_k^{(t)} = \mathbb{E} [(\tanh U^{(t)})^k]\,, \label{def:qs}
\end{align}
%
and recall the definition of the multioverlaps
%
\begin{align}\label{def:overlap}
Q_{k} = \frac{1}{n} \sum_{i=1}^{n} \sigma_i^{(1)} \cdots \sigma_i^{(k)}, \quad 	k \geq 1
\end{align}
%
% Such multi-overlaps will always appear inside Gibbs-Boltzmann expectations $\< - \>$ associated with some Hamiltonian ${\cal H}$.
where $\bsig^{(1)}, \ldots,\bsig^{(k)}$ are $k$ {\it replicas} distributed according to the product measure 
%
\begin{align}\label{productmeasure}
\biggl\{\frac{1}{{\cal Z}_{t,s;h_0,\alpha}}\exp(-\sH_{t,s; h_0,\alpha}(\ \cdot\ , \bU, \textbf{m}, \textbf{l}, \boldsymbol{\tau}))\biggr\}^{\otimes k}.
\end{align}
%
Note that, given the quenched variables, the replicas are independent . By a slight abuse of notation expectations with respect to this product measure are still denoted 
with the usual bracket $\langle - \rangle_{t,s; {h}_0, \alpha}$. With these definitions \eqref{eq:dh_ts} becomes 
%
\begin{align}\label{finalderivative}
\frac{dp_{t,s}({h}_0, \alpha)}{ds} = & -\frac{\gamma}{T}\sum_{k= 1}^{+\infty} \frac{(-1)^{k+1}}{k} \biggl\{(\tanh J)^k \mathbb{E}\langle Q_k^p\rangle_{t,s; {h}_0, \alpha}
- p \tilde{q}_k^{(t)} \mathbb{E}[\langle Q_k\rangle_{t,s; {h}_0, \alpha}]\biggr\}
\nonumber \\ &
+ \frac{\gamma p}{T}\mathbb{E} \ln \cosh U^{(t)} -\frac{\gamma}{RT} \ln \cosh \tJ
\end{align}
%

Finally, replacing \eqref{finalderivative} in \eqref{sumR}, and expanding the second and third logarithms in \eqref{sumR}, it is easy to obtain
%
\begin{align}
p_n  = {p}_{T}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0) + \frac{\gamma}{T} \sum_{t=1}^T \int_0^1 ds \ \sR_{t,s; h_0, \alpha}
+ 
\big( p_{n, 1,0}(h_0, \alpha) - p_{n, 1,0}(0, 0) \big)
\label{eq:interpolation:main2}
\end{align}
where the so-called ``remainder term '' is equal to
\begin{align}
\sR_{t,s; h_0, \alpha}
= \sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} \ \mathbb{E}  
\Big\langle (\tanh \tJ)^{k} \big(Q_{k}^{p} - q_k^{(t) p}\big) - p \,\tilde{q}_k^{(t)} \big(Q_k - q_k^{(t)} \big) \Big\rangle_{t,s; h_0, \alpha}\,. 
\label{eq:interpolation:remainder}
\end{align}
%
Equations \eqref{eq:interpolation:main2}, \eqref{eq:interpolation:remainder} form the {\it fundamental sum rule}. We note that the sum 
in \ref{eq:interpolation:remainder} is absolutely convergent since $0\leq \tanh J <1$. Indeed $\vert Q_k\vert \leq 1$, $\vert q_k\vert \leq 1$ and 
$\vert\tilde{q}_k\vert \le (\tanh J)^k$.
%

\subsection{Exploiting multioverlap concentration}\label{sec:cancelR}
%
The next step is to exploit the concentration result for the multi-overlaps which is at the heart of the replica symmetric behavior of the model. For the present model we have the GKS correlation inequalities and 
concentration of the pressure 
(see appendix \ref{sec:free_ent_conc}) and we can apply Theorem \ref{thm:over_conc_long} of Sec. \ref{sec:conc}. For completeness  we prescisely state the result to be applied presently.
%
\begin{theorem}[Multi-overlap concentration]\label{prop:conc_overlap}
For the interpolating model, all multi-overlaps \eqref{def:overlap} concentrate around their mean
$\mathbb{E}[\<Q_k\>_{t,s; h_0, \alpha}]$.
More precisely we consider the perturbed interpolating model with $\theta\in (1/2, 5/6)$, $0 < h_0 <1$ and $0<\alpha <1$. One can find a constant $C(p, J)>0$  
(depending only on $p$ and $J$) such that for any $k\geq 1$,
$0 <\underline h < \bar h < 1$, $0 < \underline \alpha <\bar \alpha<1$ we have
\begin{align}\label{concmultiover}
\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0\,\mathbb{E} \big\< \big| Q_k^p 
- \mathbb{E}[\<Q_k\>_{t,s; h_0, \alpha}]^p \big| \big\>_{t,s; h_0, \alpha} 
\leq \frac{k}{(\tanh h_1)^{k/2}} \frac{C(p, J)}{n^{1/12}}\,.
\end{align}	
\end{theorem}
%

We use this theorem to simplify the expression \eqref{eq:interpolation:main2} and \eqref{eq:interpolation:remainder} of the remainder. We have 
%
\begin{align}\label{decompo}
\sR_{t,s; h_0, \alpha}
= 
\widehat \sR_{t,s; h_0, \alpha} 
+
\mathcal{F}_{t,s; h_0, \alpha}
\end{align}
%
where
\begin{align}\label{Rhat}
 \widehat \sR_{t,s; h_0, \alpha} = \sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} \ \mathbb{E}  
\Big\langle (\tanh \tJ)^{k} \big(\mathbb{E}[\langle Q_{k}\rangle_{t,s; h_0, \alpha}]^p  - q_k^{(t) p}\big) - p \,\tilde{q}_k^{(t)} \big(\mathbb{E}[\langle Q_k\rangle_{t,s; h_0, \alpha}]  - q_k^{(t)} \big)
\end{align}
% 
and 
\begin{align}\label{F}
 \mathcal{F}_{t,s; h_0, \alpha} = \sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} (\tanh \tJ)^k \mathbb{E}\langle Q_k^p - \mathbb{E}[\langle Q_k\rangle_{t,s; h_0, \alpha}]^p\rangle_{t,s; h_0, \alpha}\,.
\end{align}
%
In Theorem \ref{prop:conc_overlap} the bound is uniform with respect to $s\in [0,1]$, $T$, and $t\in \{1, \cdots, T\}$. Therefore for any sequence $T_n$ such that $\lim_{n\to +\infty} T_n = +\infty$ we deduce for $M >1$ an arbitrary integer
%
\begin{align}
\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0 \biggl\vert \frac{1}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds\, \mathcal{F}_{t,s; h_0, \alpha}\biggr\vert 
\leq 
\frac{C(p, J)}{n^{1/12}} \sum_{k=1}^{M-1} \frac{(\tanh J)^k}{(\tanh h_1)^{k/2}} + \frac{2(\tanh J)^M}{M(1- \tanh J)}\,.
\end{align}
for any $0 <\underline h < \bar h < 1$, $0 < \underline \alpha <\bar \alpha<1$. Taking the limit $n\to +\infty$ (for fixed $M$) and $M\to +\infty$ afterwards we find
%
\begin{align}
\lim_{n\to +\infty}\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0 \biggl\vert \frac{1}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds\, \mathcal{F}_{t,s; h_0, \alpha}\biggr\vert = 0\, .
\end{align}
%
An elementary analysis argument (see Appendix \ref{elementaryapp}) then shows that one can find sequences
 $h_0^{(n)}, \alpha_0^{(n)} \to 0$ when $n\to +\infty$, such that 
%
\begin{align}\label{fluctzero}
 \lim_{n\to +\infty}\frac{1}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds\, \mathcal{F}_{t,s; h_0^{(n)}, \alpha^{(n)}} = 0\, .
\end{align}
%
Combining \eqref{eq:interpolation:main2}, \eqref{decompo}, \eqref{fluctzero} and Lemma \ref{proof:connection1} we arrive at
%
\begin{align}\label{first-simplif}
p_n  = {p}_{T_n}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0) + \frac{\gamma}{T_n} \sum_{t=1}^{T_n} \int_0^1 ds \ \widehat \sR_{t,s; h_0^{(n)}, \alpha^{(n)}} + \smallO_n(1)
\end{align}

%
% Let $k_n\in \mathbb{N}^*$ such that $k_n\to +\infty$ as $n\to +\infty$. The rate of divergence will be adjusted later on. 
% We break the sum \eqref{eq:interpolation:remainder} in two parts
% \begin{align}
%  \sR_{t,s; h_0^{(n)}, \alpha^{(n)}} = \sR_{t,s; h_0^{(n)}, \alpha^{(n)}}^{(1)} +  \sR_{t,s; h_0^{(n)}, \alpha^{(n)}}^{(2)}
% \end{align}
% where the first term is the sum over $1\leq k\leq k_n$ and the second is the sum over $k\geq k_n$. Since 
% $\vert Q_k\vert \leq 1$, $\vert q_k\vert \leq 1$ and 
% $\vert\tilde{q}_k\vert \le (\tanh J)^k$ it is clear that 
% \begin{align}
%  \sR_{t,s; h_0^{(n)}, \alpha^{(n)}}^{(2)} \leq C_2\, p (\tanh J)^{k_n}
% \end{align}
% for some numerical constant $C_2 >0$. For the terms $1\leq k\leq k_n$ we will use 
% \begin{align}\label{concmultiover2}
% \int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0\,\frac{1}{T}\sum_{t=1}^T \int_0^1\,ds\,
% \mathbb{E} \big\< \big| Q_k^p - \mathbb{E}[\<Q_k\>_{t,s; h_0, \alpha}]^p \big| \big\>_{t,s; h_0, \alpha} \leq \frac{C_p k_n^{1/2}}{n^u}
% \end{align}
% which holds because the bound \eqref{concmultiover} is uniform in $T$ and $s\in [0,1]$.
% % 
% %
% \begin{align}
% {\cal R}_{t,s;h_0,\alpha}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}}) \equiv \sum_{k=1}^{k_{\rm max}}\frac{(-1)^{k+1}}{k} \ \mathbb{E}  \Big\langle (\tanh \tJ)^{k} \big(Q_{k}^{p} - (q_k^{(t)})^p\big) - p \,\tilde{q}_k^{(t)} \big(Q_k - q_k^{(t)} \big) \Big\rangle_{t,s; h_0, \alpha}\,.
% \end{align}
% %
% Each terms $\E\<-\>$ in this sum is bounded uniformly in $k$, $t$ and $s$ and thus Theorem \ref{prop:conc_overlap} implies directly
% %
% \begin{align}
% &\int_{\underline \alpha}^{\bar \alpha} d\alpha \int_{\underline h}^{\bar h}dh_0 \Big|\frac{1}{T}\sum_{t=1}^T\int_0^1ds\Big\{{\cal R}_{t,s;h_0,\alpha}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}})- {\cal R}_{t,s;h_0,\alpha}^{(k_{\rm max})}(\{\E\<Q_{k}\>_{t,s; h_0, \alpha}\}_{k=1}^{k_{\rm max}})\Big\} \Big| =  {\cal O}(n^{-u}k_{\rm max}^{3/2})\,.\label{28}
% \end{align}
% Now choose, say, $k_{\rm max}=\Theta(\ln n)$ (many other choices are fine, as long as $n^{-u}k_{\rm max}^{3/2}\to0$ and $k_{\rm max}\to\infty$ when $n\to\infty$; the requirement that $k_{\rm max}\to\infty$ will become clear very soon). With this choice, we can assert from \eqref{28} and using Lemma \ref{elementaryapp} twice that there exists a sequence $h_n\to 0_+$ and a sub-sequence $\alpha_n=\alpha_{h_n}\to\alpha$ for any $\alpha >0$, both independent of $t$ and $s$, such that 
% %
% \begin{align}
% \lim_{n\to\infty} \Big|\frac{1}{T}\sum_{t=1}^T\int_0^1ds\Big\{ {\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}}) - {\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{\E\<Q_{k}\>_{t,s; h_n, \alpha_n}\}_{k=1}^{k_{\rm max}})\Big\} \Big| = 0\,.	\label{conc_trunc_rema}
% \end{align}
% %
% Note that for using Lemma \ref{elementaryapp} we need to make sure that the integrand is continuous. It is not difficult to show the following general fact for well-defined statistical mechanics models: For any finite $n$ the free entropy, and thus the overlaps that are related to its derivatives, are analytic; phase transitions, i.e. non-analyticity points in the free entropy where the overlaps might jump in the case of first-order transitions, can only occur in the thermodynamic limit so we are safe.  We choose these particular sequences $h_n\to0_+$, $\alpha_n\to\alpha$. Again, each terms $\E\<-\>$ in the remainder \eqref{eq:interpolation:remainder} is bounded uniformly in $n$, $t$ and $s$. The full remainder can thus be written as
% %
% \begin{align}
% {\cal R}_{t,s;h_n,\alpha_n}(\{Q_{k}\}_{k\ge1})	={\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{Q_{k}\}_{k=1}^{k_{\rm max}}) + {\cal O}\Big(\sum_{k=k_{\rm max}+1}^\infty \frac{(\tanh J)^k + \tilde{q}_k^{(t)}}{k} \Big)\,.\label{30}
% \end{align}
% %
% Note that as $U^{(t)}\sim \tilde{\sfx}^{(t)}\in \tilde{{\cal P}}$ then by definition of $\tilde{{\cal P}}$ as being the set of distributions supported on $[0,J]$ with $J>0$ fixed and of $\tilde{q}_k^{(t)}\equiv\E[(\tanh U^{(t)})^k]$, we can assert that the ${\cal O}(\cdot)$ in the last identity is a convergent sum.
% % \begin{align}
% % \sum_{k=k_{\rm max}+1}^{\infty}\frac{\tilde{q}_k^{(t)}}{k} ={\cal O}\Big(\sum_{k= k_{\rm max}+1}^\infty \frac{1}{k^{1+\epsilon}}\Big)
% % \end{align}
% % for some $\epsilon >0$ and is thus a convergent sum. 
% Recalling that $k_{\rm max}$ diverges with $n$ this sum converges to $0$ (this is the reason of the requirement that $k_{\rm max}$ is an increasing sequence with $n$) and thus the overall ${\cal O}(\cdot)$ in \eqref{30} is a $\smallO_n(1)$, where all along this paper we denote $\smallO_n(1)$ a quantity such that $\lim_{n\to\infty}\smallO_n(1)=0$ independently of everything else. The identity \eqref{30}, when combined with \eqref{conc_trunc_rema}, then implies that
% %
% \begin{align}
% &\frac{1}{T}\sum_{t=1}^T\int_0^1ds\,{\cal R}_{t,s;h_n,\alpha_n}(\{Q_{k}\}_{k\ge1})	\nonumber\\
% = &\ \frac{1}{T}\sum_{t=1}^T\int_0^1ds\,{\cal R}_{t,s;h_n,\alpha_n}^{(k_{\rm max})}(\{\E\<Q_{k}\>_{t,s; h_n, \alpha_n}\}_{k=1}^{k_{\rm max}}) + \smallO_n(1)\nonumber\\
% %
% = &\ \frac{1}{T}\sum_{t=1}^T\int_0^1ds\,\sum_{k=1}^{k_{\rm max}} \frac{(-1)^{k+1}}{k} \Big \{ (\tanh \tJ)^{k} \big( \mathbb{E}[ \< Q_{k} \>_{t,s; h_n, \alpha_n} ]^{p} - (q_k^{(t)})^p \big) \nonumber\\
% &\hspace{5cm}- p\, \tilde{q}_k^{(t)} \big( \mathbb{E} \< Q_k \>_{t,s;h_n, \alpha_n}  - q_k^{(t)} \big) \Big \} + \smallO_n(1) \,.\label{eq:interpolation:remainder:concentrated1}
%\end{align}
%

We will further simplify \eqref{first-simplif} thanks to the following crucial lemma:
%
\begin{lemma}[Weak $s$-dependence at fixed $t$]\label{lemma:weakdep}
For any $s \in [0,1]$ we have
%
\begin{align}
\big| \mathbb{E} \< Q_k \>_{t,s; h_0, \alpha_0} - \mathbb{E} \< Q_k \>_{t,0; h_0, \alpha_0} | \leq  \frac{(4p+1)\gamma n k}{T}\,.
\end{align}
%
the same inequality holds with $h_0$, $\alpha$, $T$ replaced by sequences $h_0^{(n)}$, $\alpha^{(n)}$, $T_n$.
\end{lemma}
%
\begin{proof}
The proof is immediate using an interpolation. Using the property \eqref{eq:dPoissonMean} in Appendix \ref{poisson-appendix} of Poisson distributions we find
\begin{align}
&\mathbb{E} \< Q_k \>_{t,s; h_0^{(n)}, \alpha^{(n)}}   -  \mathbb{E}\< Q_k \>_{t,0; h_0^{(n)}, \alpha^{(n)}} 
	 = \frac{1}{n} \int_{0}^{s} ds' \sum_{i=1}^{n} \frac{d}{ds'} \mathbb{E}  \< \sigma_i \>_{t,s'; {h}_n, \alpha_n}^k  \nonumber \\
	&\qquad \qquad = \frac{1}{n} \int_{0}^{s} ds' \sum_{i=1}^{n} \mathbb{E} \Big [ \frac{\gamma pk}{T} \sum_{j=1}^{n} \Big ( \< \sigma_i \>_{e_{j,s'}^{(t)} + 1}^{k-1} 
	- \< \sigma_i \>_{e_{j,s'}^{(t)}}^{k-1} \Big) - \frac{\gamma nk}{T} \Big ( \< \sigma_i \>_{m_{s'}^{(t)} + 1}^{k-1} - \< \sigma_i \>_{m_{s'}^{(t)}}^{k-1} \Big ) \Big] \,.
	\nonumber
\end{align}
From $| \< \sigma_i \> |\le 1$ we easily obtain the result. The same proof is valid with $h_0$, $\alpha$, $T$ replaced by sequences $h_0^{(n)}$, $\alpha^{(n)}$, $T_n$.
\end{proof}
%

Note that $T$ is a {\it free} parameter controlling the mean of $e_{i,s}^{(t)}$ and $m_s^{(t)}$ and can thus be set arbitrarily large. Thus we choose $T_n$ such that $n/T_n = \smallO_n(1)$. Using Lemma \ref{lemma:weakdep},  \eqref{Rhat} 
(and $\vert Q_k\vert \leq 1$, $\vert q_k\vert \leq 1$, $\vert\tilde{q}_k\vert \le (\tanh J)^k$) 
we can simplify \eqref{first-simplif} to finally obtain
%
\begin{align}\label{second-simplif}
p_n  = {p}_{T_n}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0) + \frac{\gamma}{T_n} \sum_{t=1}^{T_n}\widehat \sR_{t,0; h_0^{(n)}, \alpha^{(n)}} + \smallO_n(1)
\end{align}
%
where the remainder now takes the form
%
\begin{align}\label{Rhat-s=0}
 \widehat \sR_{t,0; h_0^{(n)}, \alpha^{(n)}} = \sum_{k=1}^{+\infty} \frac{(-1)^{k+1}}{k} \biggl\{ 
(\tanh \tJ)^{k} \big(\mathbb{E}[\langle Q_{k}\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}]^p  - q_k^{(t) p}\big) - p \,\tilde{q}_k^{(t)} \big(\mathbb{E}[\langle Q_k\rangle_{t,0; h_0^{(n)}, \alpha^{(n)}}]  - q_k^{(t)} \big)\biggr\}
\end{align}
%
Equations \eqref{second-simplif} and \eqref{Rhat-s=0} form the basis for the proof of Proposition \ref{bound2} of the next section.

%Therefore thanks to 
%Lemma~\ref{lemma:weakdep} and choosing $T\gg n k_{\rm max}$, we can remove the dependence of $\sR_{t,s; h_n, \alpha_n}$ on $s$ by re-writing \eqref{eq:interpolation:remainder:concentrated1} as
%%
%\begin{align}
%&\qquad \qquad \frac{1}{T}\sum_{t=1}^T\int_0^1ds\,{\cal R}_{t,s;h_n,\alpha_n}(\{Q_{k}\}_{k\ge1})\label{eq:interpolation:remainder:concentrated2}\\
%=& \ \frac{1}{T}\sum_{t=1}^T\sum_{k=1}^{k_{\rm max}} \frac{(-1)^{k+1}}{k} \Big \{ (\tanh \tJ)^{k} \big( \mathbb{E}[ \< Q_{k} \>_{t,0; h_n, \alpha_n} ]^{p} - (q_k^{(t)})^p \big) - p\, \tilde{q}_k^{(t)} \big( \mathbb{E} \< Q_k \>_{t,0;h_n, \alpha_n}  - q_k^{(t)} \big) \Big \} + \smallO_n(1)\,.\nonumber
%\end{align}
%%
%Lemma~\ref{thm:bd_fixed_t} is critical because $\mathbb{E}\langle Q_{p} \rangle_{t,s=0; {h}_n, \alpha_n}$ is independent of $\{ \sfx^{(t')},\tilde{\sfx}^{(t')} \}_{t' \geq t}$ an in particular of $\sfx^{(t)}$, $\tilde{\sfx}^{(t)}$ (this is only true at $s=0$ thus this specific choice). This allows an {\it adaptive} choice of \ $\tilde{\sfx}^{(t)}$ and $\sfx^{(t)}$ from $t=1$ to $T$, thus the name of the method, eventually leading to the following bounds by canceling term by term the remainder along the interpolation path.
%%%%%





==> sections/proofs.tex <==
\section{Proofs}
\label{sec:sparse:proof}





==> sections/replicasymmetricfunctionals.tex <==
\section{Replica symmetric functionals for a dilute $p$-spin ferromagnetic model}\label{replicasymmetricfunctionals}
%
As already stated in the introduction, 
one expects that multioverlap concentration
implies the validity of the replica symmetric formula. The recently developed adaptive interpolation method \cite{ourmethod} makes this implication quite transparent for a number of spin glass models
defined on dense graphs \cite{matrixfactorization}, \cite{tensorfactorization},
\cite{perceptron}, \cite{glm2layer} .
% (e.g. complete or bipartite complete graphs) coming from Bayesian inference problems which satisfy the Nishimori condition \cite{matrixfactorization}, \cite{tensorfactorization},
% \cite{perceptron}, \cite{glm2layer}. 
In Section \eqref{interpolation} we develop the adaptive interpolation method in the case of a dilute underlying graphical structure, namely the $p$-spin ferromagnetic model on a random 
Erdoes-R\'enyi hypergraph (defined in example \ref{ex1}). Then, applying the concentration results for all overlaps we prove in Section \ref{cancelling} an upper bound on the pressure that gives strong support for the direct implication between 
overlap concentration and replica symmteric formula. 
In the present Section we give the structure of the replica symmetric formulas and state our upper bound on the pressure.


% The adaptive interpolation method is well suited to explore this kind of implication as has already been shown for a number of models with a dense underlying graphical structure. 
% In Section \ref{} we develop the adaptive interpolation method for the example of the dilute $p$-spin model on a random Erdoes-R\'enyi hypergraph 
% and derive a bound which  supports this implication. This result is stated in the present section.

%
Consider the model defined in example \ref{ex1}.
The cavity method \cite{mezard1990spin} predicts that the thermodynamic limit 
of the pressure  is accessible from the following {\it replica-symmetric} functional. 
Let $\mathcal{P}$ be the set of probability measures with support on $[H, +\infty]$ and $\tilde{\cal P}$ 
the set of measures with support on $[0,J]$. 
Let $V$ be a random variable with a ``trial'' distribution $\sfx\in \mathcal{P}$ and $U$ be a ``conjugate'' random variable with a ``trial'' 
distribution $\tilde{\sfx}\in \tilde{\mathcal{P}}$. Let 
$l\sim\mathrm{Poi}(\gamma p)$ be a Poisson integer. Take $p$  i.i.d. copies of  $V$ denoted by $V_i$, $i=1, \ldots, p$ and $l$ iid copies of $U$
denoted by $U_b$, $b=1, \ldots, l$.
The {\it two letter} replica-symmetric functional is defined as (given here in two equivalent forms for later convenience)
\begin{align}\label{eq:RSFreeEntropy1}
p_{\mathrm{RS}}^{(2)} ( \sfx, \tilde{\sfx} ) 
	& = \mathbb{E} \ln \Big ( e^{H} \prod_{b=1}^{l} (1 + \tanh U_b ) + e^{-H} \prod_{b=1}^{l} (1 - \tanh U_b ) \Big) \-
	+ \gamma \mathbb{E} \ln \Big ( 1 + \tanh \tJ \prod_{i=1}^{p}\tanh V_i \Big)  \nonumber \\
	&  - p\gamma \mathbb{E} \ln \Big ( 1 + \tanh U \tanh V \Big )
	+ \gamma \ln \cosh \tJ
	\nonumber \\ &
	=
	 \mathbb{E}\ln\Big( 1 + e^{- 2(H + \sum_{b=1}^l U_b)}\Big) - \mathbb{E}\sum_{b=1}^l\ln \Big( 1 + e^{- 2 U_b}\Big)
	 + \gamma \mathbb{E} \ln \Big ( 1 + \tanh \tJ \prod_{i=1}^{p}\tanh V_i \Big)  
	 \nonumber \\ & 
	 - p\gamma \mathbb{E} \ln \Big ( 1 + \tanh U \tanh V \Big )
	+ H -\ln 2 + \gamma \ln \cosh \tJ	
\end{align}
We note for completeness that since the $U_b$'s are iid Wald's Lemma implies that the second term on the right hand side equals 
\begin{align}
 \E \sum_{b=1}^{l}\ln \Big( 1 + e^{-2 U_b}\Big) = \gamma p\E\ln \Big( 1 + e^{-2 U} \Big)
\end{align}

The stationary points of this functional satisfy the two equations 
\begin{align}
\tanh U \overset{d}{=} (\tanh \tJ) \prod_{i=1}^{p-1} \tanh V_i,  \qquad V \overset{d}{=} H + \sum_{b=1}^{l} U_b.
\label{eq:de-fixedpoint}
\end{align}
where $\overset{d}{=}$ means equality in the sense of distributions.
We define another important {\it one letter} replica-symmetric functional $p_{\rm RS}^{(1)}(\sfx)$ expressed entirely in terms of {\it one} 
distribution $\sfx\in \mathcal{P}$ . Take a trial random variable $V\sim \sfx\in \mathcal{P}$ and 
{\it define} $U$ thanks to the first equation in \eqref{eq:de-fixedpoint}
where $V_i$, $i=1, \cdots, p-1$ are i.i.d copies of $V$. Take $l\sim {\rm Poi}(\gamma p)$ i.i.d copies of $U$, labelled
$U_b$, $b=1, \cdots, l$. Then define $p_{\rm RS}^{(1)}(\sfx)$ as the right hand side of \eqref{eq:RSFreeEntropy1} where the expectation is over $V$'s and the Poisson integer $l$.

The cavity method leads to expressions for the pressure involving variational problems over the replica symmetric functionals. More precisely it is conjectured that
\begin{align}
 \lim_{n\to +\infty} p_n = {\rm extr}_{(\sfx, \tilde\sfx)\in \mathcal{P}\times \tilde{\mathcal{P}}} \,p_{\rm RS}^{(2)}(\sfx, \tilde\sfx) = \sup_{\sfx\in \mathcal{P}} p_{\rm RS}^{(1)}(\sfx)
\end{align}
No general claim about the nature of the extremum in the first equality. Here we have genuine infinite dimensional variational problems and proving the second equality between the two variational problems is also an open problem.
%This is dicussed at more length in Section \ref{willseeifwewrite}. 

%\subsection{Generalized replica symmetric functionals}

We introduce a  "generalization" of the replica symmetric functional that naturally appears in the adaptive interpolation method. 
%\begin{definition}[Generalized free entropy functional]\label{def:genpot}
Take an integer $T\geq 1$. For $t=1,\dots, T$ consider independent random variables  $V^{(t)}\sim \sfx^{(t)}\in \mathcal{P}$ 
 and $U^{(t)}\sim \tilde{\sfx}^{(t)}\in\tilde{\mathcal{P}}$ where $\sfx^{(t)}$ and $\tilde{\sfx}^{(t)}$ are trial distributions over which we shall optimize. 
We set $\underline{\sfx} = \{\sfx^{(t)}\}_{t=1}^T \in \mathcal{P}^T$ and $\underline{\tilde \sfx}= \{\tilde{\sfx^{(t)}}\}_{t=1}^T\in \tilde{\mathcal{P}}^T$. 
Let 
% $h_0$, $h_1$, $\alpha$ non-negative constants and draw independent Poisson integers $\tau \sim \mathrm{Poi}(\alpha n^{\theta-1})$,
% $\theta \in (1/2, 1)$, and 
$l^{{(t)}} \sim \mathrm{Poi}(\gamma p/T)$. 
We define the {\it two letter} generalization of the RS functional:
\begin{align}
{p}_{T}^{(2)}( \underline{\sfx}, \underline{\tilde{\sfx}}) 
	& =\E\ln \Big( e^{H} \prod_{t=1}^{T} \prod_{b=1}^{l^{(t)}} (1 + \tanh U_b^{(t)} ) + e^{-H} \prod_{t=1}^{T} \prod_{b=1}^{l^{(t)}} (1 - \tanh U_b^{(t)} ) \Big) \nonumber \\
	& \quad + \frac{\gamma}{T} \sum_{t=1}^{T} \E\ln \Big( 1 + \tanh \tJ \prod_{i=1}^{p} \tanh V_i^{(t)} \Big) \-
	 - \frac{\gamma p}{T} \sum_{t=1}^{T}\E \ln \Big( 1 + \tanh U^{(t)} \tanh V^{(t)} \Big)  + \gamma \ln \cosh \tJ
	 \nonumber \\ &
	=
	\E\ln \Big( 1 + e^{-2(H +\sum_{t=1}^{T} \sum_{b=1}^{l^{(t)}} U_b^{(t)})} \Big) - \sum_{t=1}^{T} \E \sum_{b=1}^{l^{(t)}}\ln \Big( 1 + e^{-2 U_b^{(t)}} \Big)   \nonumber \\
	& \quad + \frac{\gamma}{T} \sum_{t=1}^{T} \E\ln \Big( 1 + \tanh \tJ \prod_{i=1}^{p} \tanh V_i^{(t)} \Big) \-
	 - \frac{\gamma p}{T} \sum_{t=1}^{T}\E \ln \Big( 1 + \tanh U^{(t)} \tanh V^{(t)} \Big)  
	 \nonumber \\ &
	 \quad
	 + H -\ln 2 + \gamma \ln \cosh \tJ 
\label{eq:RSFreeEntropy_coupled1}
\end{align}
Note again that, since $U_b^{(t)}$ are iid, Wald's lemma implies the second term of the right hand side can be written as 
\begin{align}
 \sum_{t=1}^{T} \E \sum_{b=1}^{l^{(t)}}\ln \Big( 1 + e^{-2 U_b^{(t)}} \Big) = \frac{\gamma p}{T}\sum_{t=1}^{T} \E\ln \Big( 1 + e^{-2 U^{(t)}} \Big)
\end{align}
We also define a {\it one letter} version of this functional. For each $t=1, \cdots, T$ proceed as follows. Take a trial random variables $V^{(t)}\sim \sfx^{(t)}\in \mathcal{P}$ and 
{\it define} $U^{(t)}$ thanks to 
\begin{align}
 \tanh U^{(t)} \overset{d}{=} \tanh J\prod_{i=1}^{p-1} \tanh V_i^{(t)}
\end{align}
where $V_i^{(t)}$, $i=1, \cdots, p-1$ are i.i.d copies of $V^{(t)}$. Take $l^{(t)}\sim {\rm Poi}(\gamma p/T)$ i.i.d copies of $U^{(t)}$, labelled
$U_b^{(t)}$, $b=1, \cdots, l$. Then define $p_{T}^{(1)}(\underline\sfx)$ as the right hand side of \eqref{eq:RSFreeEntropy_coupled1} where the expectation is over $V$'s and the Poisson integers only.

A few remarks are in order. For $T=1$ the generalized functionals $p_T^{(2)}$, $p_T^{(1)}$ reduce to the usual RS functionals $p_{\rm RS}^{(2)}$, $p_{\rm RS}^{(1)}$. 
Also, for any $T$, the generalized functionals evaluated on the diagonal are equal to the RS functionals. 
Formally the stationary point equations for \eqref{eq:RSFreeEntropy_coupled1} are 
\begin{align}
 \tanh U^{(t)} \overset{d}{=} \tanh J\prod_{i=1}^{p-1} \tanh V_i^{(t)}, \quad V^{(t)} \overset{d}{=} \sum_{t=1}^T\sum_{b=1}^{l^{(t)}} U_b^{(t)}
\end{align}
and because of the second equation the fixed point distributions are in fact independent of $t$. This suggests that the stationary points of the generalized functionals are attained on the diagonal. Going one step further and 
assuming that the supremum of $p_T^{(1)}(\cdot)$ is not attained at the boundary of $\mathcal{P}^T$ but is attained at a stationary point, we conjecture that for all $T\geq 1$:
\begin{align}
 \sup_{\underline{\sfx}\in \mathcal{P}^T} p_T^{(1)}(\underline \sfx) = \sup_{\sfx\in \mathcal{P}}p_{\rm RS}(\sfx)
\end{align}
%Further support for this conjecture is given in section \ref{willseeifwewrite}. 

% We immediately state two useful properties.
% In Appendix \ref{proof3.3} we show
% \begin{lemma}\label{thm:connection2}
% Let $\underline{\sfx}, \underline{\tilde{\sfx}} \in \mathcal{P}^T$. For any sequence ${h}_0^{(n)} \rightarrow 0_{+}$ and $\alpha^{(n)}\to\alpha \geq 0$ we have
% \begin{align}
% \lim_{n \rightarrow \infty} \big|{p}_{T}(\underline{\sfx}, \underline{\tilde{\sfx}}; h_0^{(n)}, \alpha^{(n)}) - {p}_{T}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0)\big| = 0\,.
% \end{align}
% \end{lemma}
% %
% One can easily check that if $\sfx^{(t)} = \sfx$ and $\tilde{\sfx}^{(t)} = \tilde{\sfx}$ for all $t=1,\ldots,T$ then 
% ${p}_{{\rm RS}}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0) = p_{\mathrm{RS}}(\sfx, \tilde{\sfx})$.
% Furthermore, we show in  Appendix~\ref{proof:h_RS_coupled:equivalence} the following 
% %
% \begin{lemma}\label{lemma:3.2}
% The extremum of \eqref{eq:RSFreeEntropy_coupled1} (for $h_0=\alpha=0$) is attained on the diagonal 
% \begin{align}
% { \adjustlimits \sup_{\underline{\tilde{\sfx}} \in \tilde{\mathcal{P}}^T} \inf_{\underline{\sfx} \in \mathcal{P}^T}} 
% {p}_{T}(\underline{\sfx}, \underline{\tilde{\sfx}}; 0,0) = 
% { \adjustlimits \sup_{\tilde{\sfx} \in \mathcal{P}} \inf_{\sfx \in \mathcal{P}}} p_{\mathrm{RS}}(\sfx, \tilde{\sfx})\,.
% \label{eq:h_RS_coupled:equivalence}
% \end{align}
% An analogous statement for non zero $h_0, \alpha$ is true but will not be needed.
% %Moreover the extrema of the left hand side are attained 
% %at stationary points that satisfy ( $\overset{d}{=}$ is equality in distribution)
% %\begin{align}
% %V^{(t)} \overset{d}{=} H + \sum_{b=1}^{l^{(t)}-1} U_b^{(t)}, \quad \quad
% %\tanh U^{(t)} \overset{d}{=} (\tanh \tJ) \prod_{i=1}^{p-1} \tanh V_i^{(t)} \qquad \forall\ t=1,\dots,T
% %\label{eq:bp-update}
% %\end{align}
% %\label{thm:at-stat-pt}
% \end{lemma}
% %

We can now state our main application of multioverlap concentration.
% 
\begin{proposition}\label{bound2}
For the ferromagnetic $p$-spin model defined in example \ref{ex1} there exist a sequence $T_n\to +\infty$, $n\to +\infty$ such that
\begin{align}
p_n \leq \sup_{\underline\sfx \in \mathcal{P}^{T_n}}p_{\mathrm{T_n}}^{(1)}(\underline\sfx) + \smallO_n(1)
\end{align}
\end{proposition}
Note that if one could prove that $\sup_{\underline{\sfx}\in \mathcal{P}^T} p_T^{(1)}(\underline \sfx) \leq \sup_{\sfx\in \mathcal{P}}p_{\rm RS}(\sfx)$ (or the equality) one would deduce form this 
proposition that $\limsup_{n\to \infty} p_n\leq \sup_{\sfx\in \mathcal{P}}p_{\rm RS}(\sfx)$.

%{\color{blue}
%\subsection{Conjectures}
%
%Our main wrong result is the following:
%%
%\begin{theorem}[Replica-symmetric formula]\label{main-thm}
%For the ferromagnetic $p$-spin model defined in \eqref{eq:Gibbs}
%the thermodynamic limit of the pressure is given by:
%\begin{align}
%\lim_{n \rightarrow \infty} p_n 
%= \sup_{\sfx \in \mathcal{P}}  \inf_{\tilde{\sfx} \in \tilde{\mathcal{P}}} p_{\mathrm{RS}}(\sfx, \tilde{\sfx})\,.
%\end{align}
%\end{theorem}
%%
%This theorem follows from the two matching bounds in Propositions \ref{prop:lowerbound} and \ref{prop:upperbound} proved in Section \ref{sec:cancelR}. 
%As a byproduct of our analysis we also obtain two related propositions also proved in Section \ref{sec:cancelR}:
%%
%\begin{proposition}[Bound 1]\label{bound1}
%For the ferromagnetic $p$-spin model defined in \eqref{eq:Gibbs} we have
%\begin{align}
% \liminf_{n \rightarrow \infty} p_n \geq { \adjustlimits \sup_{\tilde{\sfx} \in \tilde{\mathcal{P}}} \inf_{\sfx \in \mathcal{P}}} p_{\mathrm{RS}}(\sfx, \tilde{\sfx})
%\end{align}
%When $p=2$ we also can show
%\begin{align}
% \limsup_{n \rightarrow \infty} p_n \leq { \adjustlimits \sup_{\tilde{\sfx} \in \tilde{\mathcal{P}}} \inf_{\sfx \in \mathcal{P}}} p_{\mathrm{RS}}(\sfx, \tilde{\sfx})
%\end{align}
%and therefore the equality holds. 
%\end{proposition}
%%
%\begin{proposition}[Bound 2]\label{bound2}
%For the ferromagnetic $p$-spin model defined in \eqref{eq:Gibbs} we have
%\begin{align}
%\limsup_{n \rightarrow \infty} p_n \leq \sup_{\sfx \in \mathcal{P}}  \tilde p_{\mathrm{RS}}(\sfx)
%\end{align}
%\end{proposition}
%%
%Let us immediately make a few remarks about these last two statements. Their proof does not use the existence of the thermodynamic limit explicitly and for this reason we express the statement 
%with liminf and limsup, although we know (e.g., from Theorem \ref{main-thm}) that the thermodynamic limit exists. More importantly we conjecture 
%that both bounds are in fact tight so the equalities hold
%\begin{align}\label{comparison}
% { \adjustlimits \sup_{\tilde{\sfx} \in \tilde{\mathcal{P}}} \inf_{\sfx \in\mathcal{P}}} p_{\mathrm{RS}}(\sfx, \tilde{\sfx}) = 
% { \adjustlimits \sup_{\sfx \in \mathcal{P}} \inf_{\tilde{\sfx} \in\tilde{\mathcal{P}}}} p_{\mathrm{RS}}(\sfx, \tilde{\sfx})
% = \sup_{\sfx \in \mathcal{P}}\tilde p_{\mathrm{RS}}(\sfx)
%\end{align}
%and that the extrema are attained at the same distributions on each side of the equality, and satisfy the equations the 
%stationary  point equations \eqref{eq:de-fixedpoint}. An argument for this conjecture comes from an explicit check
%at the level of the ferromagnetic fully connected $p$-spin model (see \cite{Barbier-macris-CW} for more details). Besides we can prove the first equality in the Ising case $p=2$. A rigorous comparison of the two variational problems 
%involved in \eqref{comparison} does not appear to be trivial for the diluted model and is not adressed in the present paper.
%}
%


